Final-state interactions in the CP asymmetries of charm-meson two-body decays

Urgent theoretical progress is needed in order to provide an estimate in the Standard Model of the recent measurement by LHCb of direct CP violation in charm-meson two-body decays. Rescattering effects must be taken into account for a meaningful theoretical description of the amplitudes involved in such category of observables, as signaled by the presence of large strong phases. We discuss the computation of the latter effects based on a two-channel coupled dispersion relation, which exploits isospin-zero phase-shifts and inelasticity parameterizations of data coming from the rescattering processes $ \pi \pi \to \pi \pi $, $ \pi K \to \pi K $, and $ \pi \pi \to K \overline{K} $. The determination of the subtraction constants of the dispersive integrals relies on the leading contributions to the transition amplitudes from the $ 1/N_C $ counting, where $N_C$ is the number of QCD colours. Furthermore, we use the measured values of the branching ratios to help in selecting the non-perturbative inputs in the isospin limit, from which we predict values for the CP asymmetries. We find that the predicted level of CP violation is much below the experimental value.

==> extrapolation.tex <==
[\textbf{note that this exercise is done in the elastic limit, in which $\delta^0_0$ is the phase-shift for pions}]

Extrapolating linearly in $s$ the parametrized phase-shift up to $m_D$ one gets: $\delta_0^2 \simeq (-41 \pm 11)^{\rm o}$ at $ s=m_D^2 $.
This can be tested against data in the following way.
The phase-shift difference
%
\begin{equation}
	\Delta = \delta^0_0 - \delta_0^2
\end{equation}
can be extracted based on an isospin analysis of branching ratios and CP asymmetries, resulting in:
%
\begin{equation}
	\Delta_\text{CKMfitter} = \pm (94 \pm 8)^{\rm o}
\end{equation}
Combining the extrapolated value of $\delta_0^2$, with the values of $\delta_0^0$, one gets: $\Delta \simeq (121 \pm 30)^{\rm o}$ for sol.~I, $\Delta \simeq (68 \pm 42)^{\rm o}$ for sol.~II, and $\Delta \simeq (112 \pm 29)^{\rm o}$ for sol.~III.
All values are compatible with $ \Delta_\text{CKMfitter} $, but uncertainties are still large. [decide on how to refer to results derived based on the use of CKMfitter: given your present plans, the best would be advertising it as future work involving all of us]

==> numerical_results.tex <==
\section*{Results from MO solution+large $ N_c $}

%individual indices: -1.9..-2.4 total (-0.79..1.05 individual)

[\textbf{have to build an intuition about Omnes matrix elements: I could plot Omnes matrix elements against the values in the integrand?; I will rather give the complex phases @ $m_D$ and indicate the inelasticity}]

[\textbf{Can use $ \Omega (m_K^2) $ to control uncertainty}][is the large modulation coming from just above the threshold? [no, rather larger energies]; note that we are not including correlations with the phase-shift: the error band in the latter is small][small modulations in the phase-shift $\delta$ at energies $\sim m_D$ (compared to the baseline of $2 \pi$ radians) have small net effects: \textit{it should not be true}, since in the elastic case we would have a factor $ \tan \delta $ in the numerator of the integrand/\textit{however, the analytic solution depends on $\delta$}!!!][not strictly true that the phase-shift does not have a large error bar!!]

Some special cases at $ m_D^2 $ and $ m_K^2 $ (solution I for $ \delta^0_0 $; subtraction at $ m_\pi^2 $; $ \eta |_{\rm lim} = 0.5 $):

\begin{itemize}
	\item[(a-I)] based on solution I for $ \eta_0^0 $, for which there is a large discontinuity of $ | g_0^0 | $ at $ 4 m_K^2 $ (solution B of $ \phi_0^0 $, solution B' of $ | g_0^0 | $) (NB: close to perfectly inelastic limit @ $ m_D $); $ \omega_\pi (m_D^2) = 0.0759+0.066 = 0.1419 $ and $ \omega_K (m_D^2) = 0.06-0.2268 = -0.1668 $; note that $ |\Omega_{1 1} (m_K^2)| = 1.50 $
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	-0.11 + 0.55 i & -0.12 - 0.69 i \\
	 0.12 - 0.54 i & -0.42 + 0.50 i \\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	 1.16 + 0.95 i & 0.16 + 0.13 i \\
	-0.01 + 0.84 i & 1.34 + 0.12 i \\
	\end{pmatrix}
\end{equation}

$ | \Omega^{(0)}_{1 1} |^2 = 0.31 \,, | \Omega^{(0)}_{1 2} |^2 = 0.49 \,, \hat{\omega}_\pi = -0.37 \,, | \Omega^{(0)}_{2 1} |^2 = 0.31 \,, | \Omega^{(0)}_{2 2} |^2 = 0.43 \,, \hat{\omega}_K = -0.32 $

	\item[(b-I)] based on solution I for $ \eta_0^0 $, for which there is a large discontinuity of $ | g_0^0 | $ at $ 4 m_K^2 $ (solution B of $ \phi_0^0 $, solution B' of $ | g_0^0 | $, with ``damping'') (NB: close to perfectly inelastic limit @ $ m_D $) %I have seen the same trend when I first did not include any info about modg00 below threshold
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	-0.12 + 0.41 i & -0.11 - 0.79 i \\
	 0.05 - 0.43 i & -0.45 + 0.59 i \\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	 1.20 + 0.98 i & 0.22 + 0.18 i \\
	-0.10 + 0.53 i & 1.27 + 0.10 i \\
	\end{pmatrix}
\end{equation}

%$ | \Omega^{(0)}_{1 1} |^2 =  \,, | \Omega^{(0)}_{1 2} |^2 =  \,, \hat{\omega}_\pi =  \,, | \Omega^{(0)}_{2 1} |^2 =  \,, | \Omega^{(0)}_{2 2} |^2 =  \,, \hat{\omega}_K =  $

	\item[(c-I)] ``interpolating'' inelasticity; $ \omega_\pi (m_D^2) = 0 + 0.1216 = 0.1216 $ and $ \omega_K (m_D^2) = 0.0252-0.1638 = -0.1386 $; note that $ |\Omega_{1 1} (m_K^2)| = 1.50 $
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	0.00 + 0.64 i & -0.19 - 0.85 i\\
	0.07 - 0.42 i & -0.39 + 0.36 i\\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	 1.17 + 0.95 i & 0.18 + 0.15 i \\
	-0.02 + 0.76 i & 1.33 + 0.12 i \\
	\end{pmatrix}
\end{equation}

$ | \Omega^{(0)}_{1 1} |^2 = 0.41 \,, | \Omega^{(0)}_{1 2} |^2 = 0.76 \,, \hat{\omega}_\pi = -0.54 \,, | \Omega^{(0)}_{2 1} |^2 = 0.18 \,, | \Omega^{(0)}_{2 2} |^2 = 0.28 \,, \hat{\omega}_K = -0.18 $

	\item[(d-I)] based on $ | g_0^0 | $, solution B$^{(')}$ (NB: close to elastic limit @ $ m_D $); $ \omega_\pi (m_D^2) = -0.3675+0.4096 = 0.0421 $ (\textbf{important cancellation for isospin-zero--only effect!}) and $ \omega_K (m_D^2) = 0.0096-0.0551 = -0.0455 $; note that $ |\Omega_{1 1} (m_K^2)| = 1.45 $
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	0.21 + 1.28 i & -0.32 - 1.75 i \\
	0.08 - 0.19 i & -0.29 + 0.12 i \\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	 1.12 + 0.91 i & 0.22 + 0.18 i \\
	-0.04 + 0.81 i & 1.38 + 0.16 i \\
	\end{pmatrix}
\end{equation}

$ | \Omega^{(0)}_{1 1} |^2 = 1.7 \,, | \Omega^{(0)}_{1 2} |^2 = 3.2 \,, \hat{\omega}_\pi = -2.3 \,, | \Omega^{(0)}_{2 1} |^2 = 0.043 \,, | \Omega^{(0)}_{2 2} |^2 = 0.098 \,, \hat{\omega}_K = -0.046 $

	\item[(e-I)] based on $ | g_0^0 | $, solution C$^{(')}$ (NB: close to elastic limit @ $ m_D $); $ \omega_\pi (m_D^2) = -0.3515+0.391 = 0.0395 $ (\textbf{important cancellation for isospin-zero--only effect!}) and $ \omega_K (m_D^2) = 0.0078-0.054 = -0.0462 $; note that $ |\Omega_{1 1} (m_K^2)| = 1.46 $
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	0.19 + 1.15 i & -0.34 - 1.85 i \\
	0.06 - 0.18 i & -0.30 + 0.13 i \\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	 1.13 + 0.92 i & 0.23 + 0.19 i \\
	-0.05 + 0.74 i & 1.36 + 0.15 i \\
	\end{pmatrix}
\end{equation}

$ | \Omega^{(0)}_{1 1} |^2 = 1.4 \,, | \Omega^{(0)}_{1 2} |^2 = 3.5 \,, \hat{\omega}_\pi = -2.2 \,, | \Omega^{(0)}_{2 1} |^2 = 0.036 \,, | \Omega^{(0)}_{2 2} |^2 = 0.11 \,, \hat{\omega}_K = -0.041 $

	\item[(f-I)] based on $ | g_0^0 | $, solution C$^{(')}$, with ``damping'' below $ 1.2 $~GeV$^2$ (NB: close to elastic limit @ $ m_D $)
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	0.13 + 0.84 i & -0.38 - 2.10 i \\
	0.01 - 0.16 i & -0.31 + 0.18 i \\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	 1.16 + 0.95 i & 0.33 + 0.27 i \\
	-0.12 + 0.46 i & 1.30 + 0.13 i \\
	\end{pmatrix}
\end{equation}

%$ | \Omega^{(0)}_{1 1} |^2 =  \,, | \Omega^{(0)}_{1 2} |^2 =  \,, \hat{\omega}_\pi =  \,, | \Omega^{(0)}_{2 1} |^2 =  \,, | \Omega^{(0)}_{2 2} |^2 =  \,, \hat{\omega}_K =  $

\end{itemize}
Note that $ \Omega_{11} \neq \Omega_{21} $, and $ \Omega_{12} \neq \Omega_{22} $, leading to a certain amount of $ SU(3) $ breaking. In the purely data-driven cases shown above (i.e., without ``damping'' or ``interpolation''), $ \Omega_{1 1} (m_K^2) = |\Omega_{1 1} (m_K^2)| \exp (i \, {\text{arg}~\Omega_{1 1} (m_K^2)} ) $ with $ |\Omega_{1 1} (m_K^2)| = (1.45 - 1.50) $ (Pallante, Pich: {\color{blue} $ \mathcal{R}_0 = 1.41 \pm 0.06 $}); $ \omega_\pi (m_K^2) = 0.1508-0.152 = -0.0012 $ (\textbf{important cancellation for isospin-zero--only effect!}, expected since in the elastic region $ \delta_2 = \delta_1 $). %and $ \omega_K (m_K^2) = -0.0012-1.1256 = -1.1268 $
%and $ {\text{arg}~\Omega_{1 1} (m_K^2)} = (39.11^{\rm o} - 39.12^{\rm o}) $ (the angle $ \delta^0_0 (m_K^2) = 39.14^{\rm o} $ -- the two must be equal by Watson's theorem (inelasticity equal to one), I attribute the small difference to numerics [note in particular I do some interpolation to find the value at $ m_K = 496 $~MeV, with points at $ 479 $~MeV and $ 506 $~MeV])

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Some special cases at $ m_D^2 $ and $ m_K^2 $ (solution II for $ \delta^0_0 $; subtraction at $ m_\pi^2 $; $ \eta |_{\rm lim} = 0.5 $): [naive extrapolation of the phase-shift from $ 1.8 $~GeV to $ 1.9 $~GeV; inelasticity contained typos]

\begin{itemize}
	\item[(a-II)] based on solution II for $ \eta_0^0 $, for which there is a large discontinuity of $ | g_0^0 | $ at $ 4 m_K^2 $ (solution B of $ \phi_0^0 $, solution B' of $ | g_0^0 | $) (NB: close to perfectly inelastic limit @ $ m_D $)
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	-0.04 + 0.43 i & -0.28 - 0.60 i \\
	 0.18 - 0.49 i & -0.51 + 0.48 i \\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	 1.16 + 0.94 i & 0.17 + 0.14 i \\
	-0.01 + 0.83 i & 1.34 + 0.12 i \\
	\end{pmatrix}
\end{equation}

$ | \Omega^{(0)}_{1 1} |^2 = 0.19 \,, | \Omega^{(0)}_{1 2} |^2 = 0.44 \,, \hat{\omega}_\pi = -0.25 \,, | \Omega^{(0)}_{2 1} |^2 = 0.27 \,, | \Omega^{(0)}_{2 2} |^2 = 0.49 \,, \hat{\omega}_K = -0.33 $

	\item[(d-II)] based on $ | g_0^0 | $, solution B$^{(')}$ (NB: close to elastic limit @ $ m_D $)
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	0.30 + 0.22 i & -0.82 - 0.48 i \\
	0.08 - 0.47 i & -0.17 + 0.40 i \\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	 1.15 + 0.93 i & 0.21 + 0.17 i \\
	-0.01 + 0.82 i & 1.36 + 0.15 i \\
	\end{pmatrix}
\end{equation}

$ | \Omega^{(0)}_{1 1} |^2 = 0.14 \,, | \Omega^{(0)}_{1 2} |^2 = 0.9 \,, \hat{\omega}_\pi = -0.35 \,, | \Omega^{(0)}_{2 1} |^2 = 0.23 \,, | \Omega^{(0)}_{2 2} |^2 = 0.19 \,, \hat{\omega}_K = -0.2 $

	\item[(e-II)] based on $ | g_0^0 | $, solution C$^{(')}$ (NB: close to elastic limit @ $ m_D $)
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	0.23 + 0.18 i & -0.87 - 0.50 i \\
	0.06 - 0.42 i & -0.17 + 0.42 i \\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	 1.15 + 0.94 i & 0.22 + 0.18 i \\
	-0.03 + 0.76 i & 1.34 + 0.14 i \\
	\end{pmatrix}
\end{equation}

$ | \Omega^{(0)}_{1 1} |^2 = 0.085 \,, | \Omega^{(0)}_{1 2} |^2 = 1. \,, \hat{\omega}_\pi = -0.29 \,, | \Omega^{(0)}_{2 1} |^2 = 0.18 \,, | \Omega^{(0)}_{2 2} |^2 = 0.21 \,, \hat{\omega}_K = -0.19 $

\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Some special cases at $ m_D^2 $ and $ m_K^2 $ (solution III for $ \delta^0_0 $; subtraction at $ m_\pi^2 $; $ \eta |_{\rm lim} = 0.5 $): [naive extrapolation of the phase-shift from $ 1.8 $~GeV to $ 1.9 $~GeV; inelasticity contained typos]

\begin{itemize}
	\item[(a-III)] based on solution III for $ \eta_0^0 $, for which there is a large discontinuity of $ | g_0^0 | $ at $ 4 m_K^2 $ (solution B of $ \phi_0^0 $, solution B' of $ | g_0^0 | $) (NB: close to perfectly inelastic limit @ $ m_D $)
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	-0.05 + 0.47 i & -0.23 - 0.64 i \\
	 0.14 - 0.45 i & -0.49 + 0.41 i \\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	 1.18 + 0.96 i & 0.14 + 0.12 i \\
	 0.00 + 0.84 i & 1.32 + 0.10 i \\
	\end{pmatrix}
\end{equation}

$ | \Omega^{(0)}_{1 1} |^2 = 0.22 \,, | \Omega^{(0)}_{1 2} |^2 = 0.46 \,, \hat{\omega}_\pi = -0.29 \,, | \Omega^{(0)}_{2 1} |^2 = 0.22 \,, | \Omega^{(0)}_{2 2} |^2 = 0.41 \,, \hat{\omega}_K = -0.25 $

	\item[(d-III)] based on $ | g_0^0 | $, solution B$^{(')}$ (NB: close to elastic limit @ $ m_D $)
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	0.77 + 2.30 i & -1.22 - 3.58 i \\
	0.28 - 0.26 i & -0.51 + 0.32 i \\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	 1.16 + 0.94 i & 0.17 + 0.14 i \\
	-0.02 + 0.83 i & 1.35 + 0.13 i \\
	\end{pmatrix}
\end{equation}

$ | \Omega^{(0)}_{1 1} |^2 = 5.9 \,, | \Omega^{(0)}_{1 2} |^2 = 14. \,, \hat{\omega}_\pi = -9.2 \,, | \Omega^{(0)}_{2 1} |^2 = 0.15 \,, | \Omega^{(0)}_{2 2} |^2 = 0.36 \,, \hat{\omega}_K = -0.23 $

	\item[(e-III)] based on $ | g_0^0 | $, solution C$^{(')}$ (NB: close to elastic limit @ $ m_D $)
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	0.66 + 1.98 i & -1.25 - 3.67 i \\
	0.22 - 0.24 i & -0.50 + 0.34 i \\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	 1.16 + 0.94 i & 0.18 + 0.15 i \\
	-0.04 + 0.76 i & 1.33 + 0.12 i \\
	\end{pmatrix}
\end{equation}

$ | \Omega^{(0)}_{1 1} |^2 = 4.4 \,, | \Omega^{(0)}_{1 2} |^2 = 15. \,, \hat{\omega}_\pi = -8.1 \,, | \Omega^{(0)}_{2 1} |^2 = 0.11 \,, | \Omega^{(0)}_{2 2} |^2 = 0.37 \,, \hat{\omega}_K = -0.19 $

\end{itemize}
In cases (d-III) and (e-III), it seems that the combination of a stronger phase-variance close to $ m_D $ and an inelasticity $ \eta \lesssim 1 $ leads to large elements of the Omnes matrix. %I had already observed a strong variation around $m_D^2$ for solution III in the elastic limit (i.e., $ \eta = 1 $), see \input{elastic_limit_ratio_pions_kaons.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Some special cases at $ m_D^2 $ and $ m_K^2 $ (solution I for $ \delta^0_0 $; subtraction at $ m_\pi^2 $; $ \eta |_{\rm lim} = 1.0 $):

\begin{itemize}
	\item[(a-I)] based on solution I for $ \eta_0^0 $, for which there is a large discontinuity of $ | g_0^0 | $ at $ 4 m_K^2 $ (solution B of $ \phi_0^0 $, solution B' of $ | g_0^0 | $); $ \omega_\pi (m_D^2) = 0.008 + 0.132 = 0.141 $ and $ \omega_K (m_D^2) = 0.174 - 0.339 = -0.164 $; note that $ |\Omega_{1 1} (m_K^2)| = 1.48 $
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	-0.01 + 0.72 i & -0.18 - 0.84 i \\
	 0.30 - 0.61 i & -0.55 + 0.59 i \\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	 1.15 + 0.93 i & 0.17 + 0.14 i \\
	-0.03 + 0.83 i & 1.35 + 0.12 i \\
	\end{pmatrix}
\end{equation}

%$ | \Omega^{(0)}_{1 1} |^2 =  \,, | \Omega^{(0)}_{1 2} |^2 =  \,, \hat{\omega}_\pi =  \,, | \Omega^{(0)}_{2 1} |^2 =  \,, | \Omega^{(0)}_{2 2} |^2 =  \,, \hat{\omega}_K =  $

\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Some special cases at $ m_D^2 $ and $ m_K^2 $ (solution I for $ \delta^0_0 $; subtraction at $ m_\pi^2 $; $ \eta |_{\rm lim} = 0.5 $): updated curve for the inelasticity

\begin{itemize}
	\item[(a-I)] based on solution I for $ \eta_0^0 $, for which there is a large discontinuity of $ | g_0^0 | $ at $ 4 m_K^2 $ (solution B of $ \phi_0^0 $, solution B' of $ | g_0^0 | $); $ \omega_\pi (m_D^2) = 0.0314 + 0.0865 = 0.1179 $ and $ \omega_K (m_D^2) = 0.012 - 0.145 = -0.138 $; note that $ |\Omega_{1 1} (m_K^2)| = 1.49 $
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	-0.03 + 0.77 i & -0.11 - 0.97 i \\
	 0.02 - 0.55 i & -0.27 + 0.50 i \\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	 1.15 + 0.94 i & 0.18 + 0.15 i \\
	-0.01 + 0.83 i & 1.35 + 0.13 i \\
	\end{pmatrix}
\end{equation}

$ | \Omega^{(0)}_{1 1} |^2 = 0.59 \,, | \Omega^{(0)}_{1 2} |^2 = 0.95 \,, \hat{\omega}_\pi = -0.74 \,, | \Omega^{(0)}_{2 1} |^2 = 0.3 \,, | \Omega^{(0)}_{2 2} |^2 = 0.32 \,, \hat{\omega}_K = -0.28 $

\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Some special cases at $ m_D^2 $ and $ m_K^2 $ (solution I for $ \delta^0_0 $; subtraction at $ m_\pi^2 $; $ \eta |_{\rm lim} = 1.0 $): updated curve for the inelasticity

%[Focus in this case first, prepare (a-I), play with uncertainties]

\begin{itemize}
	\item[{\color{blue} (a-I)}] based on solution I for $ \eta_0^0 $, for which there is a large discontinuity of $ | g_0^0 | $ at $ 4 m_K^2 $ (solution B of $ \phi_0^0 $, solution B' of $ | g_0^0 | $); $ \omega_\pi (m_D^2) = -0.0875+0.2054 = 0.1179 $ and $ \omega_K (m_D^2) = 0.126 - 0.264 = -0.138 $; note that $ |\Omega_{1 1} (m_K^2)| = 1.46 $
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	 0.07 + 1.06 i & -0.19 - 1.24 i \\
	 0.22 - 0.61 i & -0.43 + 0.58 i \\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	 1.13 + 0.92 i & 0.19 + 0.16 i \\
	-0.04 + 0.81 i & 1.37 + 0.14 i \\
	\end{pmatrix}
\end{equation}

$ | \Omega^{(0)}_{1 1} |^2 = 1.1 \,, | \Omega^{(0)}_{1 2} |^2 = 1.6 \,, \hat{\omega}_\pi = -1.3 \,, | \Omega^{(0)}_{2 1} |^2 = 0.42 \,, | \Omega^{(0)}_{2 2} |^2 = 0.52 \,, \hat{\omega}_K = -0.45 $

	\item[{\color{red} (a-I, uncs.1)}] based on solution I for $ \eta_0^0 $, for which there is a large discontinuity of $ | g_0^0 | $ at $ 4 m_K^2 $ (solution B of $ \phi_0^0 $, solution B' of $ | g_0^0 | $); $ \omega_\pi (m_D^2) = -1.5798+1.6154 = 0.0356 $ and $ \omega_K (m_D^2) = -0.0258 - 0.0153 = -0.0411 $; note that $ |\Omega_{1 1} (m_K^2)| = 1.33 $
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	 0.41 + 2.66 i & -0.61 - 3.81 i \\
	-0.04 - 0.51 i & -0.03 + 0.66 i \\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	 1.04 + 0.84 i & 0.34 + 0.28 i \\
	-0.11 + 0.74 i & 1.46 + 0.25 i \\
	\end{pmatrix}
\end{equation}

$ | \Omega^{(0)}_{1 1} |^2 = 7.2 \,, | \Omega^{(0)}_{1 2} |^2 = 15. \,, \hat{\omega}_\pi = -10. \,, | \Omega^{(0)}_{2 1} |^2 = 0.26 \,, | \Omega^{(0)}_{2 2} |^2 = 0.44 \,, \hat{\omega}_K = -0.34 $

	\item[{\color{green} (a-I, uncs.2)}] based on solution I for $ \eta_0^0 $, for which there is a large discontinuity of $ | g_0^0 | $ at $ 4 m_K^2 $ (solution B of $ \phi_0^0 $, solution B' of $ | g_0^0 | $); $ \omega_\pi (m_D^2) = 0.008+0.133 = 0.141 $ and $ \omega_K (m_D^2) = 0.172-0.337 = -0.165 $; note that $ |\Omega_{1 1} (m_K^2)| = 1.48 $
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	-0.01 + 0.72 i & -0.18 - 0.78 i \\
	 0.31 - 0.63 i & -0.54 + 0.55 i \\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	 1.15 + 0.93 i & 0.17 + 0.14 i \\
	-0.03 + 0.82 i & 1.35 + 0.12 i \\
	\end{pmatrix}
\end{equation}

$ | \Omega^{(0)}_{1 1} |^2 = 0.52 \,, | \Omega^{(0)}_{1 2} |^2 = 0.64 \,, \hat{\omega}_\pi = -0.56 \,, | \Omega^{(0)}_{2 1} |^2 = 0.49 \,, | \Omega^{(0)}_{2 2} |^2 = 0.59 \,, \hat{\omega}_K = -0.51 $

\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Some special cases at $ m_D^2 $ and $ m_K^2 $ (solution II for $ \delta^0_0 $; subtraction at $ m_\pi^2 $; $ \eta |_{\rm lim} = 1.0 $): updated curve for the inelasticity [extrapolation a la Moussallam of the phase-shift and inelasticity above $ 1.8 $~GeV; inelasticity (uncertainties) as provided by Arkaitz~Rodas]

\begin{itemize}
	\item[{\color{blue} (a-II)}] based on solution II for $ \eta_0^0 $, for which there is a large discontinuity of $ | g_0^0 | $ at $ 4 m_K^2 $ (solution B of $ \phi_0^0 $, solution B' of $ | g_0^0 | $); $ \omega_\pi (m_D^2) = -1.3809 + 1.4520 = 0.0711 $ and $ \omega_K (m_D^2) = 0.0989 - 0.1819 = -0.0830 $; note that $ |\Omega_{1 1} (m_K^2)| = 1.37 $
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	1.13 + 0.85 i & -1.71 - 1.22 i \\
	0.39 - 0.31 i & -0.60 + 0.25 i \\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	 1.06 + 0.86 i & 0.29 + 0.24 i \\
	-0.10 + 0.76 i & 1.44 + 0.21 i \\
	\end{pmatrix}
\end{equation}

$ | \Omega^{(0)}_{1 1} |^2 = 2. \,, | \Omega^{(0)}_{1 2} |^2 = 4.4 \,, \hat{\omega}_\pi = -3. \,, | \Omega^{(0)}_{2 1} |^2 = 0.25 \,, | \Omega^{(0)}_{2 2} |^2 = 0.42 \,, \hat{\omega}_K = -0.31 $

	\item[{\color{red} (a-II, uncs.1)}] based on solution II for $ \eta_0^0 $, for which there is a large discontinuity of $ | g_0^0 | $ at $ 4 m_K^2 $ (solution B of $ \phi_0^0 $, solution B' of $ | g_0^0 | $); $ \omega_\pi (m_D^2) = -6.1370 + 6.1552 = 0.0182 $ and $ \omega_K (m_D^2) = 0.0206 - 0.0417 = -0.0211 $; note that {\color{orange} $ |\Omega_{1 1} (m_K^2)| = 1.21 $}
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	2.39 + 1.63 i & -3.79 - 2.56 i \\
	0.19 - 0.14 i & -0.31 + 0.11 i \\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	0.94 + 0.76 i & 0.49 + 0.40 i \\
	-0.18 + 0.68 i & 1.56 + 0.35 i \\
	\end{pmatrix}
\end{equation}

$ | \Omega^{(0)}_{1 1} |^2 = 8.4 \,, | \Omega^{(0)}_{1 2} |^2 = 21. \,, \hat{\omega}_\pi = -13. \,, | \Omega^{(0)}_{2 1} |^2 = 0.056 \,, | \Omega^{(0)}_{2 2} |^2 = 0.11 \,, \hat{\omega}_K = -0.074 $

	\item[{\color{green} (a-II, uncs.2)}] based on solution II for $ \eta_0^0 $, for which there is a large discontinuity of $ | g_0^0 | $ at $ 4 m_K^2 $ (solution B of $ \phi_0^0 $, solution B' of $ | g_0^0 | $); $ \omega_\pi (m_D^2) = -0.6575 + 0.7612 = 0.1038 $ and $ \omega_K (m_D^2) = 0.1108 - 0.2319 = -0.1211 $; note that $ |\Omega_{1 1} (m_K^2)| = 1.40 $
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	0.76 + 0.67 i & -1.14 - 0.87 i \\
	0.44 - 0.35 i & -0.66 + 0.25 i \\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	 1.09 + 0.88 i & 0.25 + 0.20 i \\
	-0.08 + 0.78 i & 1.41 + 0.18 i \\
	\end{pmatrix}
\end{equation}

$ | \Omega^{(0)}_{1 1} |^2 = 1. \,, | \Omega^{(0)}_{1 2} |^2 = 2.1 \,, \hat{\omega}_\pi = -1.4 \,, | \Omega^{(0)}_{2 1} |^2 = 0.32 \,, | \Omega^{(0)}_{2 2} |^2 = 0.5 \,, \hat{\omega}_K = -0.38 $

\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Some special cases at $ m_D^2 $ and $ m_K^2 $ (solution III for $ \delta^0_0 $; subtraction at $ m_\pi^2 $; $ \eta |_{\rm lim} = 1.0 $): updated curve for the inelasticity [extrapolation a la Moussallam of the phase-shift and inelasticity above $ 1.8 $~GeV; inelasticity (uncertainties) as provided by Arkaitz~Rodas]

\begin{itemize}
	\item[{\color{blue} (a-III)}] based on solution III for $ \eta_0^0 $, for which there is a large discontinuity of $ | g_0^0 | $ at $ 4 m_K^2 $ (solution B of $ \phi_0^0 $, solution B' of $ | g_0^0 | $); $ \omega_\pi (m_D^2) = -1.3043 + 1.3773 = 0.0730 $ and $ \omega_K (m_D^2) = 0.0634 - 0.1486 = -0.0853 $; note that $ |\Omega_{1 1} (m_K^2)| = 1.39 $
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	1.26 + 0.64 i & -2.14 - 1.04 i \\
	0.44 - 0.20 i & -0.73 + 0.14 i \\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	 1.08 + 0.86 i & 0.27 + 0.22 i \\
	-0.09 + 0.77 i & 1.42 + 0.20 i \\
	\end{pmatrix}
\end{equation}

$ | \Omega^{(0)}_{1 1} |^2 = 2. \,, | \Omega^{(0)}_{1 2} |^2 = 5.7 \,, \hat{\omega}_\pi = -3.4 \,, | \Omega^{(0)}_{2 1} |^2 = 0.23 \,, | \Omega^{(0)}_{2 2} |^2 = 0.55 \,, \hat{\omega}_K = -0.35 $

	\item[{\color{red} (a-III, uncs.1)}] based on solution III for $ \eta_0^0 $, for which there is a large discontinuity of $ | g_0^0 | $ at $ 4 m_K^2 $ (solution B of $ \phi_0^0 $, solution B' of $ | g_0^0 | $); $ \omega_\pi (m_D^2) = -10.4508 + 10.4646 = 0.0139 $ and $ \omega_K (m_D^2) = 0.0181 - 0.0343 = -0.0161 $; note that {\color{orange} $ |\Omega_{1 1} (m_K^2)| = 1.19 $}
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	3.63 + 1.66 i & -6.31 - 2.88 i \\
	0.22 - 0.09 i & -0.38 + 0.08 i \\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	 0.92 + 0.75 i & 0.54 + 0.44 i \\
	-0.18 + 0.66 i & 1.58 + 0.39 i \\
	\end{pmatrix}
\end{equation}

%$ | \Omega^{(0)}_{1 1} |^2 =  \,, | \Omega^{(0)}_{1 2} |^2 =  \,, \hat{\omega}_\pi =  \,, | \Omega^{(0)}_{2 1} |^2 =  \,, | \Omega^{(0)}_{2 2} |^2 =  \,, \hat{\omega}_K =  $

	\item[{\color{magenta} (a-III, uncs.1')}] based on solution III for $ \eta_0^0 $, for which there is a large discontinuity of $ | g_0^0 | $ at $ 4 m_K^2 $ (solution B of $ \phi_0^0 $, solution B' of $ | g_0^0 | $); $ \omega_\pi (m_D^2) = -6.3533 + 6.3782 = 0.0249 $ and $ \omega_K (m_D^2) = 0.0415 - 0.0704 = -0.0289 $; note that {\color{orange} $ |\Omega_{1 1} (m_K^2)| = 1.26 $}
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	2.84 + 1.31 i & -4.86 - 2.23 i \\
	0.31 - 0.13 i & -0.52 + 0.13 i \\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	 0.98 + 0.79 i & 0.45 + 0.36 i \\
	-0.15 + 0.70 i & 1.53 + 0.32 i \\
	\end{pmatrix}
\end{equation}

%$ | \Omega^{(0)}_{1 1} |^2 =  \,, | \Omega^{(0)}_{1 2} |^2 =  \,, \hat{\omega}_\pi =  \,, | \Omega^{(0)}_{2 1} |^2 =  \,, | \Omega^{(0)}_{2 2} |^2 =  \,, \hat{\omega}_K =  $

	\item[{\color{magenta} (a-III, uncs.1'')}] based on solution III for $ \eta_0^0 $, for which there is a large discontinuity of $ | g_0^0 | $ at $ 4 m_K^2 $ (solution B of $ \phi_0^0 $, solution B' of $ | g_0^0 | $); $ \omega_\pi (m_D^2) = -2.9970 + 3.0415 = 0.0445 $ and $ \omega_K (m_D^2) = 0.0565 - 0.1084 = -0.0519 $; note that $ |\Omega_{1 1} (m_K^2)| = 1.34 $
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	1.92 + 0.91 i & -3.34 - 1.56 i \\
	0.39 - 0.17 i & -0.66 + 0.15 i \\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	 1.04 + 0.84 i & 0.34 + 0.28 i \\
	-0.11 + 0.75 i & 1.46 + 0.25 i \\
	\end{pmatrix}
\end{equation}

$ | \Omega^{(0)}_{1 1} |^2 = 4.5 \,, | \Omega^{(0)}_{1 2} |^2 = 14. \,, \hat{\omega}_\pi = -7.8 \,, | \Omega^{(0)}_{2 1} |^2 = 0.18 \,, | \Omega^{(0)}_{2 2} |^2 = 0.46 \,, \hat{\omega}_K = -0.28 $

	\item[{\color{green} (a-III, uncs.2)}] based on solution III for $ \eta_0^0 $, for which there is a large discontinuity of $ | g_0^0 | $ at $ 4 m_K^2 $ (solution B of $ \phi_0^0 $, solution B' of $ | g_0^0 | $); $ \omega_\pi (m_D^2) = -0.3966 + 0.5186 = 0.1220 $ and $ \omega_K (m_D^2) = 0.0758 - 0.2181 = -0.1423 $; note that $ |\Omega_{1 1} (m_K^2)| = 1.43 $
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	0.62 + 0.46 i & -1.12 - 0.64 i \\
	0.49 - 0.27 i & -0.81 + 0.15 i \\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	 1.11 + 0.90 i & 0.22 + 0.18 i \\
	-0.06 + 0.80 i & 1.39 + 0.16 i \\
	\end{pmatrix}
\end{equation}

$ | \Omega^{(0)}_{1 1} |^2 = 0.6 \,, | \Omega^{(0)}_{1 2} |^2 = 1.7 \,, \hat{\omega}_\pi = -0.99 \,, | \Omega^{(0)}_{2 1} |^2 = 0.31 \,, | \Omega^{(0)}_{2 2} |^2 = 0.68 \,, \hat{\omega}_K = -0.44 $

\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Some special cases at $ m_D^2 $ and $ m_K^2 $ (solution I for $ \delta^0_0 $; subtraction at $ m_\pi^2 $; $ \eta |_{\rm lim} = 1.0 $): updated curve for the inelasticity; $ m_\delta = 2 $ (before, it is $ m_\delta = 3 $), and $ m_\eta = 12 $

\begin{itemize}
    \item[{\color{green} (a-I, uncs.2)}] based on solution I for $ \eta_0^0 $, for which there is a large discontinuity of $ | g_0^0 | $ at $ 4 m_K^2 $ (solution B of $ \phi_0^0 $, solution B' of $ | g_0^0 | $); $ \omega_\pi (m_D^2) = $ and $ \omega_K (m_D^2) = $; note that $ |\Omega_{1 1} (m_K^2)| = 1.48 $ [I don't see much difference so I won't insist in this case, although I haven't looked at sols. II and III]
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	0.02 + 0.69 i & -0.21 - 0.76 i \\
	 0.33 - 0.58 i & -0.56 + 0.51 i \\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	 1.14 + 0.93 i & 0.18 + 0.15 i \\
	-0.04 + 0.82 i & 1.36 + 0.13 i \\
	\end{pmatrix}
\end{equation}

\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Some special cases at $ m_D^2 $ and $ m_K^2 $ (solution I for $ \delta^0_0 $; subtraction at $ m_\pi^2 $; $ \eta |_{\rm lim} = 1.0 $): updated curve for the inelasticity; $ m_\eta = 2 $ (before, it is $ m_\eta = 12 $), and $ m_\delta = 3 $

\begin{itemize}
    \item[{\color{green} (a-I, uncs.2)}] based on solution I for $ \eta_0^0 $, for which there is a large discontinuity of $ | g_0^0 | $ at $ 4 m_K^2 $ (solution B of $ \phi_0^0 $, solution B' of $ | g_0^0 | $); $ \omega_\pi (m_D^2) = $ and $ \omega_K (m_D^2) = $; note that $ |\Omega_{1 1} (m_K^2)| = 1.50 $
\begin{equation}
	\Omega (m_D^2) = \begin{pmatrix}
	-0.13 + 0.57 i & -0.10 - 0.63 i \\
	 0.12 - 0.57 i & -0.39 + 0.47 i \\
	\end{pmatrix} \,, \quad
	\Omega (m_K^2) = \begin{pmatrix}
	 1.16 + 0.95 i & 0.16 + 0.13 i \\
	0.00 + 0.84 i & 1.34 + 0.12 i \\
	\end{pmatrix}
\end{equation}

\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
	\includegraphics[scale=0.25]{inelNEW_solI.png}
	\includegraphics[scale=0.25]{inelNEW_solII.png}
	\includegraphics[scale=0.25]{inelNEW_solIII.png}
	\caption{(left) Sol.~I. (center) Sol.~II. (right) Sol.~III. ``uncs.1'' (``uncs.2'') correspond to the upper (respectively, lower) curves, shown in red (respectively, green). In the case of Sol.~III, two other curves are shown: ``{uncs.1'}'' in dashed-magenta, closer to the nominal case in blue for intermediate energies, and ``{uncs.1''}'' in dotted-magenta, closer to the nominal case in blue for larger energies.}
\end{figure}

==> old_appendices.tex <==
\section{\toni{OLD: }Decay constants and form factors}
%%%\label{app:norm_sign_convs}
%\section{Normalization and sign conventions}

%is it strictly an effective theory including charm-mesons?/$m_c$ breaking is large
%expressions for $ \overline{D}^0 $: $ D^0 $ and $ \overline{D}^0 $ do not appear in the same process, so whatever extra sign you may get for $ \overline{D}^0 $ w.r.t. $ D^0 $ gets cancelled; see proceedings by Nierste

To fix conventions, we introduce the following pseudoscalar matrix \cite{Botella:1993va} %[we will not write down the mixing term of $ \pi^0 $ and $ \eta_8 $]

\begin{equation}\label{eq:U4_U4_chiral}
	\Pi = \begin{pmatrix}
		\frac{\eta_o}{2} {\color{black} +} \frac{\pi^0}{\sqrt{2}} + \frac{\eta_8}{\sqrt{6}} + \frac{\eta_{15}}{\sqrt{12}} & \pi^+ & K^+ & \overline{D}^0 \\
		\pi^- & \frac{\eta_o}{2} {\color{black} -} \frac{\pi^0}{\sqrt{2}} + \frac{\eta_8}{\sqrt{6}} + \frac{\eta_{15}}{\sqrt{12}} & K^0 & D^- \\
		K^- & \overline{K}^0 & \frac{\eta_o}{2} - \frac{2 \, \eta_8}{\sqrt{6}} + \frac{\eta_{15}}{\sqrt{12}} & D^-_S \\
		D^0 & D^+ & D^+_S & \frac{\eta_o}{2} - \frac{3 \, \eta_{15}}{\sqrt{12}} \\
	\end{pmatrix}
\end{equation}
{\color{red} In defining like so the charge-conjugation transformations of the mesons of interest are $C(\pi^+)=\pi^-, C(\pi^0)=\pi^0, C(K^+)=K^-, C(K^0)=\overline{K}^0$.}
The chiral Noether currents of the QCD Lagrangian ($v_\mu, a_\mu, s, p$ are external Hermitian matrix-valued fields)\footnote{We will later employ in App.~\ref{app:matrix_elements} factorization for four-fermion operators, so renormalizable interactions is all we discuss at this point.}
%[need to point out what happens in presence of four-quark operators from weak interactions]

\begin{eqnarray}
    && \mathcal{L}^0_{QCD} = - \frac{1}{4} G^a_{\mu \nu} G_a^{\mu \nu} + i \bar{q}_L \gamma^\mu D_\mu q_L + i \bar{q}_R \gamma^\mu D_\mu q_R \\
	&& \mathcal{L}_{QCD} = \mathcal{L}^0_{QCD} + \bar{q} \gamma^\mu ( v_\mu + \gamma_5 a_\mu ) q - \bar{q} ( s - i \gamma_5 p ) q
\end{eqnarray}
where

\begin{equation}
	r_\mu = v_\mu + a_\mu \,, \quad \ell_\mu = v_\mu - a_\mu
\end{equation}
and of the low-energy effective chiral Lagrangian with $ U = \text{exp} \left( i \sqrt{2} \Pi / F \right) $

\begin{equation}
	\mathcal{L}_2 = \frac{1}{4} F^2 \text{Tr} \left( D_\mu U^\dagger D^\mu U + U^\dagger \chi + \chi^\dagger U \right) \,, \quad \chi = 2 B_0 ( s + i p )
\end{equation}
are related as follows \cite{Pich:1995bw}

\begin{eqnarray}
	&& (J^\mu_L)^{ij} = \bar{q}_j \gamma^\mu P_L q_i = \frac{F}{\sqrt{2}} D^\mu \Pi^{ij} - \frac{1}{2} i \left( \Pi \, \overline{D^\mu} \, \Pi \right)^{ij} + \mathcal{O} (\Pi^3 / F) \\
	&& (J^\mu_R)^{ij} = \bar{q}_j \gamma^\mu P_R q_i = - \frac{F}{\sqrt{2}} D^\mu \Pi^{ij} - \frac{1}{2} i \left( \Pi \, \overline{D^\mu} \, \Pi \right)^{ij} + \mathcal{O} (\Pi^3 / F)
\end{eqnarray}
We will only keep the leading terms below. %[explain use of $\simeq$ (note e.g. $\mathcal{O} (\Pi^3 / F)$) and systematize it; I will keep only the leading terms]

Then %[$F_\pi, F_K$ are introduced in the next section] %[an overall sign from momentum everywhere has no physical effect]

\begin{eqnarray}
	&& \langle 0 | (J^\mu_A)^{12} | \pi^+ \rangle = \langle 0 | \bar{d} \gamma^\mu \gamma_5 u | \pi^+ \rangle = - \frac{2 F}{\sqrt{2}} (-i p^\mu) \\
	%
	&& \langle 0 | (J^\mu_A)^{21} | \pi^- \rangle = \langle 0 | \bar{u} \gamma^\mu \gamma_5 d | \pi^- \rangle = \langle 0 | (J^\mu_A)^{12} | \pi^+ \rangle \\
	%
	&& \langle 0 | (J^\mu_A)^{11} | \pi^0 \rangle = \langle 0 | \bar{u} \gamma^\mu \gamma_5 u | \pi^0 \rangle = \left( {\color{black} +} \frac{1}{\sqrt{2}} \right) \langle 0 | (J^\mu_A)^{12} | \pi^+ \rangle \\
	%
	&& \langle 0 | (J^\mu_A)^{22} | \pi^0 \rangle = \langle 0 | \bar{d} \gamma^\mu \gamma_5 d | \pi^0 \rangle = \left( {\color{black} -} \frac{1}{\sqrt{2}} \right) \langle 0 | (J^\mu_A)^{12} | \pi^+ \rangle
\end{eqnarray}
we then have

\begin{eqnarray}
	&& \langle 0 | \frac{( {\color{black} +} \bar{u} u {\color{black} -} \bar{d} d )_A}{\sqrt{2}} | \pi^0 (q) \rangle = \langle 0 | ( \bar{d} u )_A | \pi^+ (q) \rangle = \langle 0 | ( \bar{u} d )_A | \pi^- (q) \rangle \\
	&& \langle 0 | {\color{black} -} ( \bar{d} d )_A | \pi^0 (q) \rangle = \langle 0 | {\color{black} +} ( \bar{u} u )_A | \pi^0 (q) \rangle \\
    && \qquad = \frac{1}{\sqrt{2}} \langle 0 | ( \bar{d} u )_A | \pi^+ (q) \rangle = \frac{1}{\sqrt{2}} \langle 0 | ( \bar{u} d )_A | \pi^- (q) \rangle \nonumber
\end{eqnarray}
also

\begin{eqnarray}
	&& 2 \, m_d \langle 0 | {\color{black} -} ( \bar{d} d )_P | \pi^0 (q) \rangle = 2 \, m_u \langle 0 | {\color{black} +} ( \bar{u} u )_P | \pi^0 (q) \rangle \\
	&& \qquad = \frac{m_d + m_u}{\sqrt{2}} \langle 0 | ( \bar{d} u )_P | \pi^+ (q) \rangle = \frac{m_d + m_u}{\sqrt{2}} \langle 0 | ( \bar{u} d )_P | \pi^- (q) \rangle \nonumber
\end{eqnarray}

\begin{eqnarray}
	&& \langle 0 | (J^\mu_A)^{13} | K^+ \rangle = \langle 0 | \bar{s} \gamma^\mu \gamma_5 u | K^+ \rangle = - \frac{2 F}{\sqrt{2}} (-i p^\mu) \\
	%
	&& \langle 0 | (J^\mu_A)^{23} | K^0 \rangle = \langle 0 | \bar{s} \gamma^\mu \gamma_5 d | K^0 \rangle = \langle 0 | (J^\mu_A)^{13} | K^+ \rangle \\
	%
	&& \langle 0 | (J^\mu_A)^{31} | K^- \rangle = \langle 0 | \bar{u} \gamma^\mu \gamma_5 s | K^- \rangle = \langle 0 | (J^\mu_A)^{13} | K^+ \rangle \\
	%
	&& \langle 0 | (J^\mu_A)^{32} | \overline{K}^0 \rangle = \langle 0 | \bar{d} \gamma^\mu \gamma_5 s | \overline{K}^0 \rangle = \langle 0 | (J^\mu_A)^{13} | K^+ \rangle
\end{eqnarray}

\begin{eqnarray}
	&& {\color{black} +} \frac{1}{\sqrt{2}} \times \langle \pi^+ | (J^\mu_V)^{41} | D^+ \rangle = {\color{black} +} \frac{1}{\sqrt{2}} \times \langle \pi^+ | \bar{u} \gamma^\mu c | D^+ \rangle \\
    && \qquad = \langle \pi^0 | (J^\mu_V)^{41} | D^0 \rangle = \langle \pi^0 | \bar{u} \gamma^\mu c | D^0 \rangle \nonumber \\
	%
	&& \langle \pi^0 | (J^\mu_V)^{42} | D^+ \rangle = \langle \pi^0 | \bar{d} \gamma^\mu c | D^+ \rangle \\
    && \qquad = {\color{black} -}\frac{1}{\sqrt{2}} \times \langle \pi^- | (J^\mu_V)^{42} | D^0 \rangle = {\color{black} -}\frac{1}{\sqrt{2}} \times \langle \pi^- | \bar{d} \gamma^\mu c | D^0 \rangle \nonumber \\
	%
	&& \langle \overline{K}^0 | (J^\mu_V)^{43} | D^+ \rangle = \langle \overline{K}^0 | \bar{s} \gamma^\mu c | D^+ \rangle = \langle K^- | (J^\mu_V)^{43} | D^0 \rangle = \langle K^- | \bar{s} \gamma^\mu c | D^0 \rangle
	%
\end{eqnarray}

We also have

\begin{eqnarray}
	&& \langle \pi^0 | ( \bar{u} c )_V | D^0 \rangle = {\color{black} +} \frac{1}{\sqrt{2}} \langle \pi^- | ( \bar{d} c )_V | D^0 \rangle \,, \\
    && (m_c-m_u) \langle \pi^0 | ( \bar{u} c )_S | D^0 \rangle = {\color{black} +} (m_c-m_d) \frac{1}{\sqrt{2}} \langle \pi^- | ( \bar{d} c )_S | D^0 \rangle
\end{eqnarray}

%\begin{equation}
%	\langle \pi^0 | ( \bar{d} c )_V | D^+ \rangle = {\color{red} -}\frac{1}{\sqrt{2}} \langle \pi^- | ( \bar{d} c )_V | D^0 \rangle \,, \quad \langle \overline{K}^0 | ( \bar{s} c )_V | D^+ \rangle = \langle K^- | ( \bar{s} c )_V | D^0 \rangle
%\end{equation}

\section{\toni{OLD:} Factorization of matrix elements}\label{app:matrix_elements}
%\section{Predictions based on large-$ N_c $; form-factors and decay constants}

%Branco et al.: ``The precision of this method is limited by the $SU(3)$-breaking effects. Although $ f_K / f_\pi $ should be the dominant $SU(3)$ breaking correction, and factorization provides a reasonable approximation for the matrix elements of the current-current operators, factorization of the matrix elements of penguin operators is questionable.''

%[\textbf{TODO:} mostly done]

Each operator in Eq.~\eqref{eq:H_eff} contributes with a tree topology with different spectator quarks; $ \langle Q_{3,5} \rangle_{tree} $ do not contribute, as $ \langle \pi^0 | ( \bar{u} u {\color{black} +} \bar{d} d )_A | 0 \rangle = 0 $.
Annihilation topology gives contributions proportional to $ M_{P_1} - M_{P_2} $ for final states $ P_1 P_2 = \pi^+ \pi^- $, $ \pi^0 \pi^0 $, $ K^+ K^- $, $ K^0 \overline{K}^0 $, $ \pi^+ \pi^0 $, $ K^+ \overline{K}^0 $.
Exchange topology gives contributions suppressed by large $ N_C $; the same for gluonic dipole insertions.
%I will not say "long-distance penguin as well", it could be interpreted wrongly
%We omit at times the final state below:
The relevant matrix elements are the following ones:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{equation}
	\langle Q_1^d \rangle_{tree; \pi^+ \pi^-} = \langle ( \bar{d} c )_{V-A} ( \bar{u} d )_{V-A} \rangle_{tree} = \langle \pi^- | ( \bar{d} c )_{V-A} | D^0 \rangle \langle \pi^+ | ( \bar{u} d )_{V-A} | 0 \rangle \\
	%&& \langle Q_1^d \rangle_{tree} = \langle ( \bar{d} c )_{V-A} ( \bar{u} d )_{V-A} \rangle_{tree} = \langle \pi^0 | ( \bar{d} c )_{V-A} | D^+ \rangle \langle \pi^+ | ( \bar{u} d )_{V-A} | 0 \rangle \nonumber
\end{equation}

\begin{equation}
	\langle Q_1^d \rangle_{tree; \pi^+ \pi^0} = {\color{black} -}\frac{1}{\sqrt{2}} \langle \pi^- | ( \bar{d} c )_{V-A} | D^0 \rangle \langle \pi^+ | ( \bar{u} d )_{V-A} | 0 \rangle
\end{equation}

%%%%

\begin{equation}
	\langle Q_2^d \rangle_{tree; \pi^0 \pi^0} = \langle ( \bar{u} c )_{V-A} ( \bar{d} d )_{V-A} \rangle_{tree} = {2 \times} \langle \pi^0 | ( \bar{u} c )_{V-A} | D^0 \rangle \langle \pi^0 | ( \bar{d} d )_{V-A} | 0 \rangle \label{eq:eq_Q2d}\\
	%&& \langle Q_2^d \rangle_{tree} = \langle ( \bar{u} c )_{V-A} ( \bar{d} d )_{V-A} \rangle_{tree} = \langle \pi^+ | ( \bar{u} c )_{V-A} | D^+ \rangle \langle \pi^0 | ( \bar{d} d )_{V-A} | 0 \rangle \nonumber
\end{equation}

\begin{equation}
	\langle Q_2^d \rangle_{tree; \pi^+ \pi^0} = {\color{black} +} \sqrt{2} \langle \pi^0 | ( \bar{u} c )_{V-A} | D^0 \rangle \langle \pi^0 | ( \bar{d} d )_{V-A} | 0 \rangle
\end{equation}

%%%%

\begin{equation}
	\langle Q_1^s \rangle_{tree; K^+ K^-} = \langle ( \bar{s} c )_{V-A} ( \bar{u} s )_{V-A} \rangle_{tree} = \langle K^- | ( \bar{s} c )_{V-A} | D^0 \rangle \langle K^+ | ( \bar{u} s )_{V-A} | 0 \rangle \\
	%&& \langle Q_1^s \rangle_{tree} = \langle ( \bar{s} c )_{V-A} ( \bar{u} s )_{V-A} \rangle_{tree} = \langle \overline{K}^0 | ( \bar{s} c )_{V-A} | D^+ \rangle \langle K^+ | ( \bar{u} s )_{V-A} | 0 \rangle \nonumber
\end{equation}

\begin{equation}
	\langle Q_1^s \rangle_{tree; K^+ \overline{K}^0} = \langle K^- | ( \bar{s} c )_{V-A} | D^0 \rangle \langle K^+ | ( \bar{u} s )_{V-A} | 0 \rangle
\end{equation}

%%%%
%the sum runs for u, d

%\begin{eqnarray}
%	&& \langle Q_3 \rangle_{tree} = \langle ( \bar{u} c )_{V-A} \Sigma_q ( \bar{q} q )_{V-A} \rangle_{tree} = \langle \pi^0 | ( \bar{u} c )_{V-A} | D^0 \rangle \langle \pi^0 | ( \bar{u} u + \bar{d} d )_{V-A} | 0 \rangle \\
%	&& \langle Q_3 \rangle_{tree} = \langle ( \bar{u} c )_{V-A} \Sigma_q ( \bar{q} q )_{V-A} \rangle_{tree} = \langle \pi^+ | ( \bar{u} c )_{V-A} | D^+ \rangle \langle \pi^0 | ( \bar{u} u + \bar{d} d )_{V-A} | 0 \rangle \nonumber
%\end{eqnarray}

%%%%
%the sum runs for u, d, s

\begin{equation}
	\langle Q_4 \rangle_{tree; \pi^+ \pi^-} = \langle \Sigma_q ( \bar{q} c )_{V-A} ( \bar{u} q )_{V-A} \rangle_{tree} = \langle \pi^- | ( \bar{d} c )_{V-A} | D^0 \rangle \langle \pi^+ | ( \bar{u} d )_{V-A} | 0 \rangle = \langle Q_1^d \rangle_{tree}
	%&& \langle Q_4 \rangle_{tree} = \langle \Sigma_q ( \bar{q} c )_{V-A} ( \bar{u} q )_{V-A} \rangle_{tree} = \langle \pi^0 | ( \bar{d} c )_{V-A} | D^+ \rangle \langle \pi^+ | ( \bar{u} d )_{V-A} | 0 \rangle \nonumber
\end{equation}

\begin{equation}
	\langle Q_4 \rangle_{tree; \pi^+ \pi^0} = {\color{black} -}\frac{1}{\sqrt{2}} \langle \pi^- | ( \bar{d} c )_{V-A} | D^0 \rangle \langle \pi^+ | ( \bar{u} d )_{V-A} | 0 \rangle
\end{equation}

%%%%

\begin{equation}
	\langle Q_4 \rangle_{tree; K^+ K^-} = \langle K^- | ( \bar{s} c )_{V-A} | D^0 \rangle \langle K^+ | ( \bar{u} s )_{V-A} | 0 \rangle = \langle Q_1^s \rangle_{tree}
	%&& \langle Q_4 \rangle_{tree} = \langle \overline{K}^0 | ( \bar{s} c )_{V-A} | D^+ \rangle \langle K^+ | ( \bar{u} s )_{V-A} | 0 \rangle \nonumber
\end{equation}

\begin{equation}
	\langle Q_4 \rangle_{tree; K^+ \overline{K}^0} = \langle K^- | ( \bar{s} c )_{V-A} | D^0 \rangle \langle K^+ | ( \bar{u} s )_{V-A} | 0 \rangle
\end{equation}

%%%%

\begin{equation}
	\langle Q_4 \rangle_{tree; \pi^0 \pi^0} = {2 \times} \langle \pi^0 | ( \bar{u} c )_{V-A} | D^0 \rangle \langle \pi^0 | ( \bar{u} u )_{V-A} | 0 \rangle = {\color{black} -} \langle Q_2^d \rangle_{tree} \label{eq:eq_Q4}
	%&& \langle Q_4 \rangle_{tree} = \langle \pi^+ | ( \bar{u} c )_{V-A} | D^+ \rangle \langle \pi^0 | ( \bar{u} u )_{V-A} | 0 \rangle \nonumber
\end{equation}

\begin{equation}
	\langle Q_4 \rangle_{tree; \pi^+ \pi^0} = {\color{black} +} \sqrt{2} \langle \pi^0 | ( \bar{u} c )_{V-A} | D^0 \rangle \langle \pi^0 | ( \bar{u} u )_{V-A} | 0 \rangle
\end{equation}

%%%%
%the sum runs for u, d, s

%\begin{eqnarray}
%	&& \langle Q_5 \rangle_{tree} = \langle ( \bar{u} c )_{V-A} \Sigma_q ( \bar{q} q )_{V+A} \rangle_{tree} = \langle \pi^0 | ( \bar{u} c )_{V-A} | D^0 \rangle \langle \pi^0 | ( \bar{u} u + \bar{d} d )_{V+A} | 0 \rangle \\
%	&& \langle Q_5 \rangle_{tree} = \langle ( \bar{u} c )_{V-A} \Sigma_q ( \bar{q} q )_{V+A} \rangle_{tree} = \langle \pi^+ | ( \bar{u} c )_{V-A} | D^+ \rangle \langle \pi^0 | ( \bar{u} u + \bar{d} d )_{V+A} | 0 \rangle \nonumber
%\end{eqnarray}

%%%%
%the sum runs for u, d, s

\begin{equation}
	\langle Q_6 \rangle_{tree; \pi^+ \pi^-} = -2 \, \langle \Sigma_q ( \bar{q} c )_{S-P} ( \bar{u} q )_{S+P} \rangle_{tree} = -2 \, \langle \pi^- | ( \bar{d} c )_{S-P} | D^0 \rangle \langle \pi^+ | ( \bar{u} d )_{S+P} | 0 \rangle \\
	%&& \langle Q_6 \rangle_{tree} = -2 \, \langle \Sigma_q ( \bar{q} c )_{S-P} ( \bar{u} q )_{S+P} \rangle_{tree} = -2 \, \langle \pi^0 | ( \bar{d} c )_{S-P} | D^+ \rangle \langle \pi^+ | ( \bar{u} d )_{S+P} | 0 \rangle \nonumber
\end{equation}

\begin{equation}
	\langle Q_6 \rangle_{tree; \pi^+ \pi^0} = {\color{black} +}2 \, \frac{1}{\sqrt{2}} \langle \pi^- | ( \bar{d} c )_{S-P} | D^0 \rangle \langle \pi^+ | ( \bar{u} d )_{S+P} | 0 \rangle
\end{equation}

%%%%

\begin{equation}
	\langle Q_6 \rangle_{tree; K^+ K^-} = -2 \, \langle K^- | ( \bar{s} c )_{S-P} | D^0 \rangle \langle K^+ | ( \bar{u} s )_{S+P} | 0 \rangle \\
	%&& \langle Q_6 \rangle_{tree} = -2 \, \langle \overline{K}^0 | ( \bar{s} c )_{S-P} | D^+ \rangle \langle K^+ | ( \bar{u} s )_{S+P} | 0 \rangle \nonumber
\end{equation}

\begin{equation}
	\langle Q_6 \rangle_{tree; K^+ \overline{K}^0} = -2 \, \langle K^- | ( \bar{s} c )_{S-P} | D^0 \rangle \langle K^+ | ( \bar{u} s )_{S+P} | 0 \rangle
\end{equation} 

%%%%

\begin{equation}
	\langle Q_6 \rangle_{tree; \pi^0 \pi^0} = - {2 \times} 2 \, \langle \pi^0 | ( \bar{u} c )_{S-P} | D^0 \rangle \langle \pi^0 | ( \bar{u} u )_{S+P} | 0 \rangle \label{eq:eq_Q6}\\
	%&& \langle Q_6 \rangle_{tree} = -2 \, \langle \pi^+ | ( \bar{u} c )_{S-P} | D^+ \rangle \langle \pi^0 | ( \bar{u} u )_{S+P} | 0 \rangle \nonumber
\end{equation}

\begin{equation}
	\langle Q_6 \rangle_{tree; \pi^+ \pi^0} = {\color{black} -} 2 \, \sqrt{2} \langle \pi^0 | ( \bar{u} c )_{S-P} | D^0 \rangle \langle \pi^0 | ( \bar{u} u )_{S+P} | 0 \rangle
\end{equation}
The extra factor of $ {2} $ in Eqs.~\eqref{eq:eq_Q2d}, \eqref{eq:eq_Q4}, \eqref{eq:eq_Q6} comes from identical particles in the final state.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For the form factors, we have ($ q = p_D - p_P $), $ x = d, s $, with kinematic constraint $ f^{D P}_+ (0) = f^{D P}_0 (0) $
%[likely, lattice references consider $ | D^+ \rangle = | c \bar{d} \rangle $, $ | D^0 \rangle = | c \bar{u} \rangle $, $ | \overline{K}^0 \rangle = | s \bar{d} \rangle $, $ | K^- \rangle = | s \bar{u} \rangle $, $ | \pi^- \rangle = | d \bar{u} \rangle $; I can't however decide on what lattice would take for $ | \pi^0 \rangle = \pm \frac{| d \bar{d} \rangle - | u \bar{u} \rangle}{\sqrt{2}} $?] I included the section of SU(4)xSU(4)
%[what if $ P = \pi^0 $?; in FLAG they say $ x = d, s $/not enough to conclude there is no $ \pi^0 $, and in fact there is]

\begin{equation}
	\langle P | ( \bar{x} c )_{V} | D \rangle = f^{D P}_+ (q^2) \left( {p_D}_\mu + {p_P}_\mu - \frac{M_D^2 - M_P^2}{q^2} q_\mu \right) + f^{D P}_0 (q^2) \frac{M_D^2 - M_P^2}{q^2} q_\mu
\end{equation}
%A part vanishes
and thus %[sign difference?, problem when comparing to Toni?/agrees w/ Schacht+]

\begin{equation}
	\langle P | ( \bar{x} c )_{S} | D \rangle = f^{D P}_0 (q^2) \frac{M_D^2 - M_P^2}{m_c - m_x}
\end{equation}

%\LVS{We assume that the values of $ f^{D \pi}_+, f^{D \pi}_0 $ given by Lattice calculations correspond to the flavours $ D^0, \pi^- $. [necessary to say?: these are isospin breaking corrections]}

For the decay constants (compared to App.~\ref{app:norm_sign_convs}, $ \sqrt{2} \, F = f $, and $f_\pi \neq f_K$ integrate further corrections)
%[likely, lattice references consider $ | \pi^+ \rangle = | u \bar{d} \rangle $ and $ | K^+ \rangle = | u \bar{s} \rangle $] I included the section of SU(4)xSU(4) %(the sign of the RH side flips when taking the complex conjugate; it is a global sign without practical effect) %[necessary, otherwise contracting and taking hermitian conjugate would not commute]

\begin{equation}
	\langle 0 | ( \bar{d} u )_A | \pi^+ (q) \rangle = i q_\mu f_{\pi^+} \,, \quad \langle 0 | ( \bar{s} u )_A | K^+ (q) \rangle = i q_\mu f_{K^+}
\end{equation}
and thus	

\begin{equation}
	\langle 0 | ( \bar{d} u )_P | \pi^+ (q) \rangle = -i \frac{M_\pi^2}{m_u + m_d} f_{\pi^+} \,, \quad \langle 0 | ( \bar{s} u )_P | K^+ (q) \rangle = -i \frac{M_K^2}{m_u + m_s} f_{K^+}
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Then:

\begin{equation}
	\langle Q_1^d \rangle_{tree; \pi^+ \pi^-} = \langle Q_4 \rangle_{tree; \pi^+ \pi^-} = i f_{\pi^+} f^{D \pi}_0 (M_\pi^2) (M_D^2 - M_\pi^2)
\end{equation}

\begin{equation}
	\langle Q_1^s \rangle_{tree; K^+ K^-} = \langle Q_4 \rangle_{tree; K^+ K^-} = i f_{K^+} f^{D K}_0 (M_K^2) (M_D^2 - M_K^2)
\end{equation}

\begin{eqnarray}
	&& \langle Q_6 \rangle_{tree; \pi^+ \pi^-} = -2 i f_{\pi^+} \frac{M_\pi^2}{m_u + m_d} f^{D \pi}_0 (M_\pi^2) \frac{M_D^2 - M_\pi^2}{m_c - m_d} \\
    && \qquad = -2 \frac{M_\pi^2}{m_u + m_d} \frac{1}{m_c - m_d} \langle Q_4 \rangle_{tree; \pi^+ \pi^-} \nonumber
\end{eqnarray}

\begin{eqnarray}
	&& \langle Q_6 \rangle_{tree; K^+ K^-} = -2 i f_{K^+} \frac{M_K^2}{m_u + m_s} f^{D K}_0 (M_K^2) \frac{M_D^2 - M_K^2}{m_c - m_s} \\
    && \qquad = -2 \frac{M_K^2}{m_u + m_s} \frac{1}{m_c - m_s} \langle Q_4 \rangle_{tree; K^+ K^-} \nonumber
\end{eqnarray}
The relative minus sign implies a cancellation among $ \langle Q_6 \rangle_{tree} $ and $ \langle Q_4 \rangle_{tree} $ (because their Wilson coefficients carry the same sign, see App.~\ref{app:num_inputs}).
Note that, at $ m_c \sim 1.3~\text{GeV} $:

\begin{equation}\label{eq:r_values}
	\frac{M_\pi^2}{m_u + m_d} \frac{1}{m_c - m_d} \simeq \frac{M_K^2}{m_u + m_s} \frac{1}{m_c - m_s} \simeq 2
\end{equation}
(not being then a sizable source of breaking of a potential symmetry relating pion and kaon channels).
%showing that $ m_c $ is comparable to $ v_{\langle \bar{q} q \rangle_0}/f_\pi^2 $, where $ -v_{\langle \bar{q} q \rangle_0} $ is the quark condensate

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Finally:

\begin{equation}
	{\color{black} -} \langle Q_2^d \rangle_{tree; \pi^0 \pi^0} = \langle Q_4 \rangle_{tree; \pi^0 \pi^0} = {\color{black} +} {2 \times} \frac{1}{2} \langle Q_1^d \rangle_{tree; \pi^+ \pi^-} = {\color{black} +} {2 \times} \frac{1}{2} \langle Q_4 \rangle_{tree; \pi^+ \pi^-}
\end{equation}

\begin{equation}
	\langle Q_6 \rangle_{tree; \pi^0 \pi^0} = {\color{black} +} {2 \times} \frac{1}{2} \frac{m_c-m_d}{m_c-m_u} \frac{m_u+m_d}{2 \, m_u} \langle Q_6 \rangle_{tree; \pi^+ \pi^-}
\end{equation}

%[move to conventions only]
%\input{conventions.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

With the necessary elements dully provided, we then define, see Eq.~\eqref{eq:H_eff}:

\begin{eqnarray}
    && T^{CC}_{\pi^+ \pi^-} = -i G_F \, C_1 \, \lambda_d \, \langle Q_1^d \rangle_{tree; \pi^+ \pi^-} \\
    && T^{CC}_{\pi^0 \pi^0} = -i \frac{G_F}{\sqrt{2}} \, C_2 \, \lambda_d \, \langle Q_2^d \rangle_{tree; \pi^0 \pi^0} \\
    && T^{CC}_{K^+ K^-} = -i G_F \, C_1 \, \lambda_s \, \langle Q_1^s \rangle_{tree; K^+ K^-} \\
    && T^{CC}_{K^0 \overline{K}^0} = 0 \\
    && T^{P}_{\pi^+ \pi^-} = i G_F \, \lambda_b \left( C_4 \, \langle Q_4 \rangle_{tree; \pi^+ \pi^-} + C_6 \, \langle Q_6 \rangle_{tree; \pi^+ \pi^-} \right) \\
    && T^{P}_{\pi^0 \pi^0} = i \frac{G_F}{\sqrt{2}} \, \lambda_b \left( C_4 \, \langle Q_4 \rangle_{tree; \pi^0 \pi^0} + C_6 \, \langle Q_6 \rangle_{tree; \pi^0 \pi^0} \right) \\
    && T^{P}_{K^+ K^-} = i G_F \, \lambda_b \left( C_4 \, \langle Q_4 \rangle_{tree; K^+ K^-} + C_6 \, \langle Q_6 \rangle_{tree; K^+ K^-} \right) \\
    && T^{P}_{K^0 \overline{K}^0} = 0
\end{eqnarray}
where charged particles are to be taken as identical, see App.~\ref{app:isospin_decomposition}.

We consider the isospin limit, setting $ m_u, m_d \to \hat{m} $, see Tab.~\ref{tab:WCs}.

\section{\toni{OLD:} Isospin decomposition} %%%\label{app:isospin_decomposition}

%[\textbf{TODO:} discuss CPV in the charged decay mode (never discussed in the literature?) $D^+ \to \pi^+ \pi^0$; comments in personal notes]

The decomposition into states of definite isospin for pion pairs gives, employing the sign convention of Wigner \cite{Workman:2022ynf}:\footnote{Let $ \pi' $ be a triplet of $ SU(2) $

\begin{equation}
	\pi' =
	\begin{pmatrix}
	{\color{black} -} \pi_1 \\
	\pi_2 \\
	\pi_3 \\
	\end{pmatrix}
\end{equation}
which transforms as $ \pi' \to U \pi' $ in the spin-$1$ representation.
Alternatively, write the triplet as a $ 2 \times 2 $ traceless matrix

\begin{equation}
	\pi =
	\begin{pmatrix}
	{\color{black} +} \pi_2 / \sqrt{2} & \pi_1 \\
	\pi_3 & {\color{black} -} \pi_2 / \sqrt{2} \\
	\end{pmatrix}
\end{equation}
which transforms as $ \pi \to U \pi U^\dagger $ in the spin-$1/2$ representation, cf. Eq.~\eqref{eq:U4_U4_chiral}. Note the sign in front of $ \pi_1 $. The matrix $ U = 1 + i (\theta_1 T_1 + \theta_2 T_2 + \theta_3 T_3) $, with $ T_1, T_2, T_3 $ accordingly in the doublet or triplet representations.

We also identify the doublets $ \begin{pmatrix} K^+ \\ K^0 \\ \end{pmatrix} $ and $ \begin{pmatrix} \overline{D}^0 \\ D^- \\ \end{pmatrix} $, together with $ \begin{pmatrix} {\color{black} -} \overline{K}^0 \\ K^- \\ \end{pmatrix} = -i \sigma_2 \begin{pmatrix} K^+ \\ K^0 \\ \end{pmatrix}^\dagger $ and  $ \begin{pmatrix} {\color{black} -} D^+ \\ D^0 \\ \end{pmatrix} = -i \sigma_2 \begin{pmatrix} \overline{D}^0 \\ D^- \\ \end{pmatrix}^\dagger $.}

\begin{eqnarray}
	&& {\color{black} -} \langle \pi^+ \pi^- |_{id} = \sqrt{\frac{1}{3}} \langle 2\pi, I=2,M=0 | + \sqrt{\frac{2}{3}} \langle 2\pi, I=0,M=0 | \,, \\
	&& \langle \pi^0 \pi^0 | = \sqrt{\frac{2}{3}} \langle 2\pi, I=2,M=0 | - \sqrt{\frac{1}{3}} \langle 2\pi, I=0,M=0 |
\end{eqnarray}

\begin{eqnarray}
	&& \langle 2\pi, I=0,M=0 | = {\color{black} -} \sqrt{\frac{2}{3}} \langle \pi^+ \pi^- |_{id} - \sqrt{\frac{1}{3}} \langle \pi^0 \pi^0 | \,, \\
	&& \langle 2\pi, I=2,M=0 | = {\color{black} -} \sqrt{\frac{1}{3}} \langle \pi^+ \pi^- |_{id} + \sqrt{\frac{2}{3}} \langle \pi^0 \pi^0 |
\end{eqnarray}
The state $ \langle 2\pi, I=1,M=0 | = (\langle \pi^+_1 \pi^-_2 | - \langle \pi^-_1 \pi^+_2 |) / \sqrt{2} $ is not available by Bose-Einstein symmetry. We denote $ \langle \pi^+ \pi^- |_{id} = (\langle \pi^+_1 \pi^-_2 | + \langle \pi^-_1 \pi^+_2 |) / \sqrt{2} $, where the subscript ``id'' means that the $ \pi^\pm $ in $ \langle \pi^+ \pi^- |_{id} $ are to be taken as identical.

We will be denoting ($ T $ is the transition matrix):

\begin{eqnarray}
    && \langle 0 |T| D^0 \rangle = \langle 0 |T^{(1/2)}| D^0 \rangle = \mathcal{A}^\pi_0 + i \mathcal{B}^\pi_0 \\
    && \langle 2 |T^{(3/2)}| D^0 \rangle = \mathcal{A}^\pi_2 + i {\color{black} \mathcal{B}^\pi_2}
\end{eqnarray}
where $ \langle 2\pi, I=0,M=0 | \equiv \langle 0 | $ and $ \langle 2\pi, I=2,M=0 | \equiv \langle 2 | $, and $ \langle 2 |T| D^0 \rangle = \langle 2 |T^{(3/2)}| D^0 \rangle + \langle 2 |T^{(5/2)}| D^0 \rangle $. We will be neglecting $ \Delta I = 5/2 $ contributions.

Then

\begin{eqnarray}
	&& {\color{black} -} \langle \pi^+ \pi^- |_{id} T| D^0 \rangle = \sqrt{\frac{1}{3}} (\mathcal{A}^\pi_2 + i {\color{black} \mathcal{B}^\pi_2}) + \sqrt{\frac{2}{3}} ( \mathcal{A}^\pi_0 + i \mathcal{B}^\pi_0 ) \,, \\
	&& \langle \pi^0 \pi^0 |T| D^0 \rangle = \sqrt{\frac{2}{3}} (\mathcal{A}^\pi_2 + i {\color{black} \mathcal{B}^\pi_2}) - \sqrt{\frac{1}{3}} ( \mathcal{A}^\pi_0 + i \mathcal{B}^\pi_0 )
\end{eqnarray}

\begin{eqnarray}
	&& \langle 0 |T| D^0 \rangle = {\color{black} -} \sqrt{\frac{2}{3}} \langle \pi^+ \pi^- |_{id} T| D^0 \rangle - \sqrt{\frac{1}{3}} \langle \pi^0 \pi^0 |T| D^0 \rangle \,, \\
	&& \langle 2 |T| D^0 \rangle = {\color{black} -} \sqrt{\frac{1}{3}} \langle \pi^+ \pi^- |_{id} T| D^0 \rangle + \sqrt{\frac{2}{3}} \langle \pi^0 \pi^0 |T| D^0 \rangle
\end{eqnarray}

Also,

\begin{equation}
    \langle \pi^+ \pi^0 |_{id} T| D^+ \rangle = \langle \pi^+ \pi^0 |_{id} T^{(3/2)}| D^+ \rangle + \langle \pi^+ \pi^0 |_{id} T^{(5/2)}| D^+ \rangle
\end{equation}
with

\begin{equation}
	{\color{black} -} \langle \pi^+ \pi^0 |_{id} = {\color{black} -} \frac{1}{\sqrt{2}} ( \langle \pi^+_1 \pi^0_2 | + \langle \pi^0_1 \pi^+_2 | ) = \langle 2 \pi, 2, 1 |
\end{equation}

From Eckart-Wigner theorem, we have the following relation: %(the pre-factors are inverses of Clebsch-Gordan elements)

\begin{eqnarray}
	&& \sqrt{\frac{4}{3}} \langle 2, +1 | T^{(3/2)} | 1/2, + 1/2 \rangle = \sqrt{2} \langle 2,  0 | T^{(3/2)} | 1/2, - 1/2 \rangle %\\
	%&& - \sqrt{3}  \langle 2, +1 | T^{(5/2)} | 1/2, + 1/2 \rangle = \sqrt{2} \langle 2,  0 | T^{(5/2)} | 1/2, - 1/2 \rangle \nonumber
\end{eqnarray}
and thus

\begin{equation}
	{\color{black} -} \langle \pi^+ \pi^0 |_{id} T | 1/2, + 1/2 \rangle = {\color{black}{\color{black} +}} \langle \pi^+ \pi^0 |_{id} T | D^+ \rangle = \sqrt{\frac{3}{2}} (\mathcal{A}^\pi_2 + i {\color{black} \mathcal{B}^\pi_2})
\end{equation}
where we allow for a possibly non-vanishing $\mathcal{B}^\pi_2$ amplitude.
%[$\mathcal{B}^\pi_2$ depends on a single weak phase, the one of $\lambda_d$; suppose that $\mathcal{A}^\pi_2$ and $\mathcal{B}^\pi_2$ have different strong phases: then I could have CPV that would depend on the phase of $\lambda_d$ only, which is not rephasing-invariant?, so I can't have different strong phases?, true, they have the same leading $1/N_c$ expressions, when neglecting the contributions from penguin operators][if I have rescattering, I can possibly also have $\lambda_s$; note that two kaons do not form a state of total isospin-2; I could have an extra pair of pions (Bose-Einstein would not forbid having a total isospin-2)]
The dynamics of having contributions to $\mathcal{B}^\pi_2$ due to rescattering effects, making the process inelastic and introducing CP violation in this system, even in the isospin-conserving limit, will be discussed in a forthcoming publication \cite{PSVS_Ieq2:2023}.
%[relating the discussion about $G_4$ with $B_2^\pi$ is a good insight: we would indeed require some dynamics in $G_4$ (assuming the isospin-2 phase-shift does not flip value; I am overlooking $G_3$ (Leutwyler \cite{Leutwyler:2002hm} discusses P-wave, while here we are discussing S-wave)), which impacts the discussion of $D^+ \to \pi^+ \pi^0$; we are playing safe, however, because $A_2^\pi$ is being extracted from the branching ratio $D^+ \to \pi^+ \pi^0$, for which $B_2^\pi$ is irrelevant; see Donoghue, Gasser, Leutwyler on glueballs \cite{Donoghue:1990xh}]

For kaons:

\begin{eqnarray}
	&& \langle K^+_1 K^-_2 | = \frac{1}{\sqrt{2}} ( \langle 2K, 1, 0; 1/2_{\bar{s}} \; 1/2_s | + \langle 2K, 0, 0; 1/2_{\bar{s}} \; 1/2_s | ) \,, \\
%	&& \langle K^+ K^- |_{id} = \frac{1}{\sqrt{2}} ( \langle K^+ K^- | + \langle K^- K^+ | ) = \langle 2K, I = 0, M = 0 | + \langle 2K, I = 1, M = 0 | \,, \\ %NOT WELL NORMALIZED
	&& {\color{black} -} \langle K^0_1 \overline{K}^0_2 | = \frac{1}{\sqrt{2}} ( \langle 2K, 1, 0; 1/2_{\bar{s}} \; 1/2_s | - \langle 2K, 0, 0; 1/2_{\bar{s}} \; 1/2_s | )
%	&& \langle K^0 \bar{K}^0 |_{id} = \frac{1}{\sqrt{2}} ( \langle K^0 \bar{K}^0 | + \langle \bar{K}^0 K^0 | ) = - \langle 2K, I = 0, M = 0 | + \langle 2K, I = 1, M = 0 | \nonumber %NOT WELL NORMALIZED
\end{eqnarray}

\begin{eqnarray}
	&& \langle K^-_1 K^+_2 | = \frac{1}{\sqrt{2}} ( \langle 2K, 1, 0; 1/2_s \; 1/2_{\bar{s}} | - \langle 2K, 0, 0; 1/2_s \; 1/2_{\bar{s}} | ) \,, \\
	&& {\color{black} -} \langle \overline{K}^0_1 K^0_2 | = \frac{1}{\sqrt{2}} ( \langle 2K, 1, 0; 1/2_s \; 1/2_{\bar{s}} | + \langle 2K, 0, 0; 1/2_s \; 1/2_{\bar{s}} | )
\end{eqnarray}
which correspond to two possible additions of the kaon doublets.
\LVS{The first case (i.e., $1/2_{\bar{s}} \; 1/2_s$) would imply a negative sign in the off diagonal elements of Eq.~\eqref{eq:T00_expression}, while the second (i.e., $1/2_s \; 1/2_{\bar{s}}$) implies the positive sign displayed therein.} %[XCHECK which convention we are using; overall/relative sign?]
We recall the general rule for Clebsch-Gordan coefficients: %[manifests Bose symmetry]

\begin{equation}
	\langle j_1 j_2 m_1 m_2 | j_1 j_2 J M \rangle = (-1)^{J - j_1 - j_2} \langle j_2 j_1 m_2 m_1 | j_2 j_1 J M \rangle
\end{equation}
%%Then:

%\begin{eqnarray}
%	&& \langle K^+_1 K^-_2 | ( T | D^0 \rangle )_{\bar{s} s} = \frac{1}{\sqrt{2}} ( \langle 2K, 1, 0; 1/2_{\bar{s}} \; 1/2_s | ( T | D^0 \rangle )_{\bar{s} s} + \langle 2K, 0, 0; 1/2_{\bar{s}} \; 1/2_s | ( T | D^0 \rangle )_{\bar{s} s} ) \,, \nonumber\\
%	&& {\color{black} -} \langle K^0_1 \bar{K}^0_2 | ( T | D^0 \rangle )_{\bar{s} s} = \frac{1}{\sqrt{2}} ( \langle 2K, 1, 0; 1/2_{\bar{s}} \; 1/2_s | ( T | D^0 \rangle )_{\bar{s} s} - \langle 2K, 0, 0; 1/2_{\bar{s}} \; 1/2_s | ( T | D^0 \rangle )_{\bar{s} s} ) \nonumber
%\end{eqnarray}
%%\begin{eqnarray}
%%	&& \langle K^+_1 K^-_2 | ( T | D^0 \rangle )_{\bar{s} s} = \frac{1}{\sqrt{2}} ( \langle 2K, 1, 0; 1/2_s \; 1/2_{\bar{s}} | ( T | D^0 \rangle )_{s \bar{s}} - \langle 2K, 0, 0; 1/2_s \; 1/2_{\bar{s}} | ( T | D^0 \rangle )_{s \bar{s}} ) \,, \nonumber\\
%%	&& {\color{black} -} \langle K^0_1 \overline{K}^0_2 | ( T | D^0 \rangle )_{\bar{s} s} = \frac{1}{\sqrt{2}} ( \langle 2K, 1, 0; 1/2_s \; 1/2_{\bar{s}} | ( T | D^0 \rangle )_{s \bar{s}} + \langle 2K, 0, 0; 1/2_s \; 1/2_{\bar{s}} | ( T | D^0 \rangle )_{s \bar{s}} ) \nonumber
%%\end{eqnarray}

%\begin{eqnarray}
%	&& \langle K^-_1 K^+_2 | ( T | D^0 \rangle )_{s \bar{s}} = \frac{1}{\sqrt{2}} ( \langle 2K, 1, 0; 1/2_{\bar{s}} \; 1/2_s | ( T | D^0 \rangle )_{\bar{s} s} + \langle 2K, 0, 0; 1/2_{\bar{s}} \; 1/2_s | ( T | D^0 \rangle )_{\bar{s} s} ) \,, \nonumber\\
%	&& {\color{black} -} \langle \bar{K}^0_1 K^0_2 | ( T | D^0 \rangle )_{s \bar{s}} = \frac{1}{\sqrt{2}} ( \langle 2K, 1, 0; 1/2_{\bar{s}} \; 1/2_s | ( T | D^0 \rangle )_{\bar{s} s} - \langle 2K, 0, 0; 1/2_{\bar{s}} \; 1/2_s | ( T | D^0 \rangle )_{\bar{s} s} ) \nonumber
%\end{eqnarray}
%%\begin{eqnarray}
%%	&& \langle K^-_1 K^+_2 | ( T | D^0 \rangle )_{s \bar{s}} = \frac{1}{\sqrt{2}} ( \langle 2K, 1, 0; 1/2_s \; 1/2_{\bar{s}} | ( T | D^0 \rangle )_{s \bar{s}} - \langle 2K, 0, 0; 1/2_s \; 1/2_{\bar{s}} | ( T | D^0 \rangle )_{s \bar{s}} ) \,, \nonumber\\
%%	&& {\color{black} -} \langle \overline{K}^0_1 K^0_2 | ( T | D^0 \rangle )_{s \bar{s}} = \frac{1}{\sqrt{2}} ( \langle 2K, 1, 0; 1/2_s \; 1/2_{\bar{s}} | ( T | D^0 \rangle )_{s \bar{s}} + \langle 2K, 0, 0; 1/2_s \; 1/2_{\bar{s}} | ( T | D^0 \rangle )_{s \bar{s}} ) \nonumber
%%\end{eqnarray}

\noindent
We now define the symmetric combinations: %%(we now drop the subscript of $T | D^0 \rangle$)

%\begin{eqnarray}
%	&& \frac{\langle K^+_1 K^-_2 | T | D^0 \rangle + \langle K^-_1 K^+_2 | T | D^0 \rangle}{\sqrt{2}} = \langle 2K, 1, 0; 1/2_{\bar{s}} \; 1/2_s | T | D^0 \rangle + \langle 2K, 0, 0; 1/2_{\bar{s}} \; 1/2_s | T | D^0 \rangle \,, \nonumber\\
%	&& {\color{black} -} \frac{\langle K^0_1 \bar{K}^0_2 | T | D^0 \rangle + \langle \bar{K}^0_1 K^0_2 | T | D^0 \rangle}{\sqrt{2}} = \langle 2K, 1, 0; 1/2_{\bar{s}} \; 1/2_s | T | D^0 \rangle - \langle 2K, 0, 0; 1/2_{\bar{s}} \; 1/2_s | T | D^0 \rangle \nonumber
%\end{eqnarray}
\begin{eqnarray}
	&& \frac{\langle K^+_1 K^-_2 | T | D^0 \rangle + \langle K^-_1 K^+_2 | T | D^0 \rangle}{\sqrt{2}} \\
    && \qquad = \langle 2K, 1, 0; 1/2_s \; 1/2_{\bar{s}} | T | D^0 \rangle - \langle 2K, 0, 0; 1/2_s \; 1/2_{\bar{s}} | T | D^0 \rangle \,,  \nonumber\\
	&& {\color{black} -} \frac{\langle K^0_1 \overline{K}^0_2 | T | D^0 \rangle + \langle \overline{K}^0_1 K^0_2 | T | D^0 \rangle}{\sqrt{2}} \\
    && \qquad = \langle 2K, 1, 0; 1/2_s \; 1/2_{\bar{s}} | T | D^0 \rangle + \langle 2K, 0, 0; 1/2_s \; 1/2_{\bar{s}} | T | D^0 \rangle \nonumber
\end{eqnarray}

Introduce now:

%\begin{eqnarray}
%    && \langle 2K, 0, 0; 1/2_{\bar{s}} \; 1/2_s | T | D^0 \rangle = \langle 2K, 0, 0; 1/2_{\bar{s}} \; 1/2_s | T^{(1/2)} | D^0 \rangle = \mathcal{A}^K_0 + i \mathcal{B}^K_0 \\
%    && \langle 2K, 1, 0 | T | D^0 \rangle = \langle 2K, 1, 0 | T^{(1/2)} | D^0 \rangle + \langle 2K, 1, 0 | T^{(3/2)} | D^0 \rangle \\
%    && \langle 2K, 1, 0; 1/2_{\bar{s}} \; 1/2_s | T^{(1/2)} | D^0 \rangle = \mathcal{A}^K_{11} + i \mathcal{B}^K_{11} \\
%    && \langle 2K, 1, 0; 1/2_{\bar{s}} \; 1/2_s | T^{(3/2)} | D^0 \rangle = \mathcal{A}^K_{13} + i {\color{black} \mathcal{B}^K_{13}}
%\end{eqnarray}
\begin{eqnarray}
    && \langle 2K, 0, 0; 1/2_s \; 1/2_{\bar{s}} | T | D^0 \rangle = \langle 2K, 0, 0; 1/2_s \; 1/2_{\bar{s}} | T^{(1/2)} | D^0 \rangle = \mathcal{A}^K_0 + i \mathcal{B}^K_0 \\
    && \langle 2K, 1, 0 | T | D^0 \rangle = \langle 2K, 1, 0 | T^{(1/2)} | D^0 \rangle + \langle 2K, 1, 0 | T^{(3/2)} | D^0 \rangle \\
    && \langle 2K, 1, 0; 1/2_s \; 1/2_{\bar{s}} | T^{(1/2)} | D^0 \rangle = \mathcal{A}^K_{11} + i \mathcal{B}^K_{11} \\
    && \langle 2K, 1, 0; 1/2_s \; 1/2_{\bar{s}} | T^{(3/2)} | D^0 \rangle = \mathcal{A}^K_{13} + i {\color{black} \mathcal{B}^K_{13}}
\end{eqnarray}
With that, we write:

%\begin{eqnarray}
%	&& \langle K^+ K^- |_{id} T| D^0 \rangle = (\mathcal{A}^K_0 + i \mathcal{B}^K_0) + (\mathcal{A}^K_{11} + i \mathcal{B}^K_{11}) + (\mathcal{A}^K_{13} + i {\color{black} \mathcal{B}^K_{13}}) \\
%	&& {\color{black} -} \langle K^0 \bar{K}^0 |_{id} T| D^0 \rangle = - (\mathcal{A}^K_0 + i \mathcal{B}^K_0) + (\mathcal{A}^K_{11} + i \mathcal{B}^K_{11}) + (\mathcal{A}^K_{13} + i {\color{black} \mathcal{B}^K_{13}})
%\end{eqnarray}
\begin{eqnarray}
	&& \langle K^+ K^- |_{id} T| D^0 \rangle = - (\mathcal{A}^K_0 + i \mathcal{B}^K_0) + (\mathcal{A}^K_{11} + i \mathcal{B}^K_{11}) + (\mathcal{A}^K_{13} + i {\color{black} \mathcal{B}^K_{13}}) \\
	&& {\color{black} -} \langle K^0 \overline{K}^0 |_{id} T| D^0 \rangle = (\mathcal{A}^K_0 + i \mathcal{B}^K_0) + (\mathcal{A}^K_{11} + i \mathcal{B}^K_{11}) + (\mathcal{A}^K_{13} + i {\color{black} \mathcal{B}^K_{13}})
\end{eqnarray}

From Eckart-Wigner:

\begin{eqnarray}
	&& - \sqrt{4} \langle 1, +1 | T^{(3/2)} | 1/2, + 1/2 \rangle = \sqrt{2} \langle 1,  0 | T^{(3/2)} | 1/2, - 1/2 \rangle \\
	&& \langle 1, +1 | T^{(1/2)} | 1/2, + 1/2 \rangle = \sqrt{2} \langle 1,  0 | T^{(1/2)} | 1/2, - 1/2 \rangle %=\sqrt{2} \langle 0,  0 | T^{(1/2)} | 1/2, - 1/2 \rangle, NOT FROM Wigner-Eckart
\end{eqnarray}
Since:

\begin{equation}
	{\color{black} -} \langle K^+_1 \overline{K}^0_2 | = \langle 2 K, 1, 1; 1/2_{\bar{s}} \; 1/2_s |
%	{\color{red} \langle K^+ \bar{K}^0 |_{id} = \frac{1}{\sqrt{2}} ( \langle K^+ \bar{K}^0 | + \langle \bar{K}^0 K^+ | ) = \sqrt{2} \langle 2 K, 1, 1 | } %NOT WELL NORMALIZED
\end{equation}
and thus

\begin{equation}
	\langle K^+ \overline{K}^0 |_{id} T | D^+ \rangle = 2 ( \mathcal{A}^K_{11} + i \mathcal{B}^K_{11} ) - (\mathcal{A}^K_{13} + i {\color{black} \mathcal{B}^K_{13}})
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Physical kaons}\label{app:physical_kaons}

We have the following reciprocal states \cite{Branco:1999fs}:

\begin{equation}
	\langle K_L | = \frac{1}{2 p_K} \langle K^0 | + \frac{1}{2 q_K} \langle \overline{K}^0 | \,, \quad \langle K_S | = \frac{1}{2 p_K} \langle K^0 | - \frac{1}{2 q_K} \langle \overline{K}^0 |
\end{equation}
To leading order in weak interactions:

\begin{eqnarray}
	\langle K^+ \overline{K}^0 | T | D^+ \rangle = \langle K^+ | \otimes \left( \langle K_L | - \langle K_S | \right) q_K T | D^+ \rangle \\
	0 \sim \langle K^+ K^0 | T | D^+ \rangle = \langle K^+ | \otimes \left( \langle K_L | + \langle K_S | \right) p_K T | D^+ \rangle
\end{eqnarray}
then

\begin{eqnarray}
	&& \langle K^+ K_L | T | D^+ \rangle \simeq \frac{\langle K^+ \overline{K}^0 | T | D^+ \rangle}{2 q_K} \,,\; \langle K^- K_L | T | D^- \rangle \simeq \frac{\langle K^- K^0 | T | D^- \rangle}{2 p_K} \\
	&& \langle K^+ K_S | T | D^+ \rangle \simeq -\frac{\langle K^+ \overline{K}^0 | T | D^+ \rangle}{2 q_K} \,,\; \langle K^- K_S | T | D^- \rangle \simeq \frac{\langle K^- K^0 | T | D^- \rangle}{2 p_K}
\end{eqnarray}
Similarly

\begin{eqnarray}
	\langle K^0 \overline{K}^0 | T | D^0 \rangle = \left( \langle K_L | + \langle K_S | \right) p_K \otimes \left( \langle K_L | - \langle K_S | \right) q_K T | D^0 \rangle \\
	\langle \overline{K}^0 K^0 | T | D^0 \rangle = \left( \langle K_L | - \langle K_S | \right) q_K \otimes \left( \langle K_L | + \langle K_S | \right) p_K T | D^0 \rangle \\
	0 \sim \langle K^0 K^0 | T | D^0 \rangle = \left( \langle K_L | + \langle K_S | \right) p_K \otimes \left( \langle K_L | + \langle K_S | \right) p_K T | D^0 \rangle \\
	0 \sim \langle \overline{K}^0 \overline{K}^0 | T | D^0 \rangle = \left( \langle K_L | - \langle K_S | \right) q_K \otimes \left( \langle K_L | - \langle K_S | \right) q_K T | D^0 \rangle
\end{eqnarray}
then

\begin{equation}
	\frac{\sqrt{2}}{2 p_K q_K} \langle K^0 \overline{K}^0 |_{id} T | D^0 \rangle = \left( \langle K_L K_L | - \langle K_S K_S | \right) T | D^0 \rangle \,,\; 0 \sim \left( \langle K_L K_L | + \langle K_S K_S | \right) T | D^0 \rangle
\end{equation}

\begin{equation}
	\left( \frac{\langle K_S K_L | + \langle K_L K_S |}{\sqrt{2}} \right) T | D^0 \rangle \sim 0 \sim \left( \frac{\langle K_S K_L | + \langle K_L K_S |}{\sqrt{2}} \right) T | \overline{D}^0 \rangle
\end{equation}
and

\begin{eqnarray}
	&& \langle K_L K_L | T | D^0 \rangle \simeq \frac{\sqrt{2}}{4 p_K q_K} \langle K^0 \overline{K}^0 |_{id} T | D^0 \rangle \simeq -\langle K_S K_S | T | D^0 \rangle \\
	&& \langle K_L K_L | T | \overline{D}^0 \rangle \simeq \frac{\sqrt{2}}{4 p_K q_K} \langle K^0 \overline{K}^0 |_{id} T | \overline{D}^0 \rangle \simeq -\langle K_S K_S | T | \overline{D}^0 \rangle
\end{eqnarray}
where we make use of the symmetrized combination %[\textbf{note the normalization}: agrees with the previous section]

\begin{equation}
	\langle K^0 \overline{K}^0 |_{id} = \frac{\langle K^0 \overline{K}^0 | + \langle \overline{K}^0 K^0 |}{\sqrt{2}}
\end{equation}
already introduced above.
We have that: $ | p_K |^2 = (1 + \delta) / 2 $, $ | q_K |^2 = (1 - \delta) / 2 $; $ | \delta | \ll 1 $ and is neglected.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Simplified expressions}\label{app:simplified_expressions}

For illustrative purposes only,
we give expressions valid in the limits $ M_\pi^2 / M_D^2 $, $ M_K^2 / M_D^2 \to 0^+ $ ($ m_u / m_c $, $ m_d / m_c $, $ m_s / m_c \to 0^+ $), $ f_K / f_\pi $, $ F^{D K}_0 (0) / F^{D \pi}_0 (0) \to 1 $ (both ratios being in reality $\simeq 1.2$), and $ \text{Re} \{ \lambda_b \} \to 0 $ (since $ | \lambda_b | $ is rephasing invariant, and much smaller than $ | \lambda_d |, | \lambda_s | $):

%%%%%%%%%%%%%%%%%%%%%%%%

\begin{equation}
	\mathcal{A}^\pi_0 \simeq - \frac{f_\pi G_F M_D^2 F^{D \pi}_0 (0)}{\sqrt{6}} \left[ (2 C_1 - C_2) \, \Omega^{(0)}_{1 1} \, \text{Re} \{ \lambda_d \} + \frac{\sqrt{3}}{\sqrt{2}} \, C_1 \, \Omega^{(0)}_{1 2} \, \text{Re} \{ \lambda_s \} \right]
\end{equation}

\begin{eqnarray}
	&& \mathcal{B}^\pi_0 \simeq - \frac{f_\pi G_F M_D^2 F^{D \pi}_0 (0)}{\sqrt{6}} \left[ (2 C_1 - C_2) \, \Omega^{(0)}_{1 1} \, \text{Im} \{ \lambda_d \} + \frac{\sqrt{3}}{\sqrt{2}} \, C_1 \, \Omega^{(0)}_{1 2} \, \text{Im} \{ \lambda_s \} \right. \\
    && \qquad\qquad\quad \left. - \frac{\sqrt{3}}{\sqrt{2}} \, ( C_4 - C_6 \, \delta^\pi_6 ) \, (\Omega^{(0)}_{1 2} + \sqrt{6} \, \Omega^{(0)}_{1 1}) \, \text{Im} \{ \lambda_b \} \right] \nonumber
\end{eqnarray}

%%%%%%%%%%%%%%%%%%%%%%%%

\begin{equation}
	\mathcal{A}^K_0 \simeq - \frac{f_K G_F M_D^2 F^{D K}_0 (0)}{\sqrt{6}} \left[ (2 C_1 - C_2) \, \Omega^{(0)}_{2 1} \, \text{Re} \{ \lambda_d \} + \frac{\sqrt{3}}{\sqrt{2}} \, C_1 \, \Omega^{(0)}_{2 2} \, \text{Re} \{ \lambda_s \} \right]
\end{equation}

\begin{eqnarray}
	&& \mathcal{B}^K_0 \simeq - \frac{f_K G_F M_D^2 F^{D K}_0 (0)}{\sqrt{6}} \left[ (2 C_1 - C_2) \, \Omega^{(0)}_{2 1} \, \text{Im} \{ \lambda_d \} + \frac{\sqrt{3}}{\sqrt{2}} \, C_1 \, \Omega^{(0)}_{2 2} \, \text{Im} \{ \lambda_s \} \right. \\
    && \qquad\qquad\quad \left. - \frac{\sqrt{3}}{\sqrt{2}} \, ( C_4 - C_6 \, \delta^K_6 ) \, (\Omega^{(0)}_{2 2} + \sqrt{6} \, \Omega^{(0)}_{2 1}) \, \text{Im} \{ \lambda_b \} \right] \nonumber
\end{eqnarray}

%%%%%%%%%%%%%%%%%%%%%%%%

\begin{equation}
	\mathcal{A}^\pi_2 \simeq - \frac{f_\pi G_F M_D^2 F^{D \pi}_0 (0)}{\sqrt{3}} \, (C_1 + C_2) \, |\Omega^{(2)}| e^{i \phi_2} \, \text{Re} \{ \lambda_d \}
\end{equation}

\begin{equation}
	\mathcal{B}^\pi_2 \simeq - \frac{f_\pi G_F M_D^2 F^{D \pi}_0 (0)}{\sqrt{3}} \, (C_1 + C_2) \, |\Omega^{(2)}| e^{i \phi_2} \, \text{Im} \{ \lambda_d \}
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%

\begin{equation}
	\mathcal{A}^K_{11} \simeq \frac{f_K G_F M_D^2 F^{D K}_0 (0)}{2} \, C_1 \, |\Omega^{(1)}| e^{i \phi_1} \, \text{Re} \{ \lambda_s \}
\end{equation}

\begin{equation}
	\mathcal{B}^K_{11} \simeq \frac{f_K G_F M_D^2 F^{D K}_0 (0)}{2} \, |\Omega^{(1)}| e^{i \phi_1} \left[ C_1  \, \text{Im} \{ \lambda_s \} - ( C_4 - C_6 \, \delta^K_6 )  \, \text{Im} \{ \lambda_b \} \right]
\end{equation}

%where $R_{\pi, K}$ are the expressions seen in Eq.~\eqref{eq:r_values}: $ R_\pi \equiv \frac{2 M_\pi^2}{2 \, \hat{m} \, (m_c - \hat{m})} $, $ R_K \equiv \frac{2 M_K^2}{(m_s + \hat{m}) \, (m_c - m_s)} $.

%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{equation}
%	\tan \arg \mathcal{A}^\pi_0 \simeq \frac{\sqrt{2} \, (2 C_1 - C_2) \, \text{Im} [ \Omega_{1 1} ] \, \text{Re} \{ \lambda_d \} + \sqrt{3} \, C_1 \, \text{Im} [ \Omega_{1 2} ] \, \text{Re} \{ \lambda_s \}}{\sqrt{2} \, (2 C_1 - C_2) \, \text{Re} [ \Omega_{1 1} ] \, \text{Re} \{ \lambda_d \} + \sqrt{3} \, C_1 \, \text{Re} [ \Omega_{1 2} ] \, \text{Re} \{ \lambda_s \}}
%\end{equation}

%\begin{eqnarray}
%	&& \qquad\qquad\quad \tan \arg \mathcal{B}^\pi_0 \simeq \\
%    && \frac{\sqrt{2} \, (2 C_1 - C_2) \, \text{Im} [ \Omega_{1 1} ] \, \text{Im} \{ \lambda_d \} + \sqrt{3} \, C_1 \, \text{Im} [ \Omega_{1 2} ] \, \text{Im} \{ \lambda_s \} - \sqrt{3} \, C_4 \, (\sqrt{6} \text{Im} [ \Omega_{1 1} ] + \text{Im} [ \Omega_{1 2} ]) \, \text{Im} \{ \lambda_b \}}{\sqrt{2} \, (2 C_1 - C_2) \, \text{Re} [ \Omega_{1 1} ] \, \text{Im} \{ \lambda_d \} + \sqrt{3} \, C_1 \, \text{Re} [ \Omega_{1 2} ] \, \text{Im} \{ \lambda_s \} - \sqrt{3} \, C_4 \, (\sqrt{6} \text{Re} [ \Omega_{1 1} ] + \text{Re} [ \Omega_{1 2} ]) \, \text{Im} \{ \lambda_b \}} \nonumber
%\end{eqnarray}

%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{equation}
%	\tan \arg \mathcal{A}^K_0 \simeq \frac{\sqrt{2} \, (2 C_1 - C_2) \, \text{Im} [ \Omega_{2 1} ] \, \text{Re} \{ \lambda_d \} + \sqrt{3} \, C_1 \, \text{Im} [ \Omega_{2 2} ] \, \text{Re} \{ \lambda_s \}}{\sqrt{2} \, (2 C_1 - C_2) \, \text{Re} [ \Omega_{2 1} ] \, \text{Re} \{ \lambda_d \} + \sqrt{3} \, C_1 \, \text{Re} [ \Omega_{2 2} ] \, \text{Re} \{ \lambda_s \}}
%\end{equation}

%\begin{eqnarray}
%	&& \qquad\qquad\quad \tan \arg \mathcal{B}^K_0 \simeq \\
%    && \frac{\sqrt{2} \, (2 C_1 - C_2) \, \text{Im} [ \Omega_{2 1} ] \, \text{Im} \{ \lambda_d \} + \sqrt{3} \, C_1 \, \text{Im} [ \Omega_{2 2} ] \, \text{Im} \{ \lambda_s \} - \sqrt{3} \, C_4 \, (\sqrt{6} \text{Im} [ \Omega_{2 1} ] + \text{Im} [ \Omega_{2 2} ]) \, \text{Im} \{ \lambda_b \}}{\sqrt{2} \, (2 C_1 - C_2) \, \text{Re} [ \Omega_{2 1} ] \, \text{Im} \{ \lambda_d \} + \sqrt{3} \, C_1 \, \text{Re} [ \Omega_{2 2} ] \, \text{Im} \{ \lambda_s \} - \sqrt{3} \, C_4 \, (\sqrt{6} \text{Re} [ \Omega_{2 1} ] + \text{Re} [ \Omega_{2 2} ]) \, \text{Im} \{ \lambda_b \}} \nonumber
%\end{eqnarray}

%%%%%%%%%%%%%%%%%%%%%%%%

%\noindent
%where
%$\mathcal{Y} = \mathcal{A}, \mathcal{B}$ with respectively $\text{X} = \text{Re}, \text{Im}$;
%$ P $ stands for $ \pi $ or $ K $.

%\input{numerical_results.tex}

==> table_Omnes.tex <==
\begin{sidewaystable}
%\begin{table}[]
    \centering
    \renewcommand{\arraystretch}{1.6}
    \begin{tabular}{|c|c|c|c|}
    \hline
         & sol.~I & sol.~II & sol.~III \\
    \hline\hline %called (a, uncs.2)
        $ - \delta \eta^0_0 $, $ m^\ast_\eta = 2 $ & $ \mathbf{ \Omega (m_D^2) = \begin{pmatrix}
	-0.13+0.57 i & -0.1-0.63 i \\
 0.12\, -0.57 i & -0.39+0.47 i \\
	\end{pmatrix} } $
        & $ \Omega (m_D^2) = \begin{pmatrix}
	0.29 + 0.48 i & -0.64 - 0.67 i \\
	0.23 - 0.54 i & -0.45 + 0.47 i \\
	\end{pmatrix} $
        & $ \Omega (m_D^2) = \begin{pmatrix}
	0.10 + 0.34 i & -0.53 - 0.51 i \\
	0.20 - 0.43 i & -0.52 + 0.36 i \\
	\end{pmatrix} $ \\
%    \hline\hline %called (a, uncs.1)
%        $ + \delta \eta^0_0 $, $ m^\ast_\eta = 12 $ & $ \Omega (m_D^2) = \begin{pmatrix}
%	 0.41 + 2.66 i & -0.61 - 3.81 i \\
%	-0.04 - 0.51 i & -0.03 + 0.66 i \\
%	\end{pmatrix} $
%        & $ \Omega (m_D^2) = \begin{pmatrix}
%	2.39 + 1.63 i & -3.79 - 2.56 i \\
%	0.19 - 0.14 i & -0.31 + 0.11 i \\
%	\end{pmatrix} $
%        & $ \Omega (m_D^2) = \begin{pmatrix}
%	3.63 + 1.66 i & -6.31 - 2.88 i \\
%	0.22 - 0.09 i & -0.38 + 0.08 i \\
%	\end{pmatrix} $ \\
%    \hline %called (a)
%        $ \eta^0_0 $, $ m^\ast_\eta = 12 $ & $ \Omega (m_D^2) = \begin{pmatrix}
%	 0.07 + 1.06 i & -0.19 - 1.24 i \\
%	 0.22 - 0.61 i & -0.43 + 0.58 i \\
%	\end{pmatrix} $
%        & $ \Omega (m_D^2) = \begin{pmatrix}
%	1.13 + 0.85 i & -1.71 - 1.22 i \\
%	0.39 - 0.31 i & -0.60 + 0.25 i \\
%	\end{pmatrix} $
%        & $ \Omega (m_D^2) = \begin{pmatrix}
%	1.26 + 0.64 i & -2.14 - 1.04 i \\
%	0.44 - 0.20 i & -0.73 + 0.14 i \\
%	\end{pmatrix} $ \\
    \hline %called (a, uncs.2)
        $ - \delta \eta^0_0 $, $ m^\ast_\eta = 6 $ & $ \Omega (m_D^2) = \begin{pmatrix}
	-0.07 + 0.65 i & -0.14 - 0.71 i \\
	0.22 - 0.60 i & -0.46 + 0.52 i \\
	\end{pmatrix} $
        & $ \Omega (m_D^2) = \begin{pmatrix}
	0.51 + 0.58 i & -0.87 - 0.77 i \\
	0.34 - 0.48 i & -0.55 + 0.40 i \\
	\end{pmatrix} $
        & $ \Omega (m_D^2) = \begin{pmatrix}
	0.33 + 0.41 i & -0.78 - 0.58 i \\
	0.35 - 0.38 i & -0.66 + 0.30 i \\
	\end{pmatrix} $ \\
    \hline %called (a, uncs.2)
        $ - \delta \eta^0_0 $, $ m^\ast_\eta = 12 $ & $ \Omega (m_D^2) = \begin{pmatrix}
	-0.01 + 0.72 i & -0.18 - 0.78 i \\
	 0.31 - 0.63 i & -0.54 + 0.55 i \\
	\end{pmatrix} $
        & $ \Omega (m_D^2) = \begin{pmatrix}
	0.76 + 0.67 i & -1.14 - 0.87 i \\
	0.44 - 0.35 i & -0.66 + 0.25 i \\
	\end{pmatrix} $
        & $ \Omega (m_D^2) = \begin{pmatrix}
	0.62 + 0.46 i & -1.12 - 0.64 i \\
	0.49 - 0.27 i & -0.81 + 0.15 i \\
	\end{pmatrix} $ \\
    \hline\hline %called (d)
        sol.~B': $ | g^0_0 | $ & $ \Omega (m_D^2) = \begin{pmatrix}
	0.36+1.98 i & -0.47-2.42 i \\
	0.35-0.12 i & -0.54+0.05 i \\
	\end{pmatrix} $
        & $ \Omega (m_D^2) = \begin{pmatrix}
	1.58+1.08 i & -2.31-1.55 i \\
	0.30-0.07 i & -0.44-0.07 i \\
	\end{pmatrix} $
        & $ \Omega (m_D^2) = \begin{pmatrix}
	2.00+0.92 i & -3.24-1.46 i \\
	0.35+0.01 i & -0.55-0.15 i \\
	\end{pmatrix} $ \\
    \hline %called (e)
        sol.~C': $ | g^0_0 | $ & $ \Omega (m_D^2) = \begin{pmatrix}
	0.34+1.80 i & -0.50-2.60 i \\
    0.31-0.13 i & -0.56+0.08 i \\
	\end{pmatrix} $
        & $ \Omega (m_D^2) = \begin{pmatrix}
	1.50+1.00 i & -2.60-1.70 i \\
    0.28-0.07 i & -0.49-0.05 i \\
	\end{pmatrix} $
        & $ \Omega (m_D^2) = \begin{pmatrix}
	1.90+0.87 i & -3.60-1.60 i \\
    0.32-0.01 i & -0.60-0.12 i \\
	\end{pmatrix} $ \\
    \hline
    \end{tabular}
    \caption{... [sols. II and III for eta are wrong!]}
    \label{tab:num_sols_Omnes}
%\end{table}
\end{sidewaystable}

==> table_WCs_masses.tex <==
\begin{table}[t]
	\centering
	\begin{tabular}{|c|c|c|c|c|c|c|}
	\hline
	% &
	%$ \mu $ & $ z_1 $ & $ z_2 $ & $ v_3 $ & $ v_4 $ & $ v_5 $ & $ v_6 $ \\ %& $ C_{8g} $
	$ \mu $ & $ C_1 $ & $ C_2 $ & $ C_3 $ & $ C_4 $ & $ C_5 $ & $ C_6 $ \\ %& $ C_{8g} $
	\hline
	%\hline
	%[Brod et al.] & $ m_c $ & $ 1.21 $ & $ -0.41 $ & $ 0.02 $ & $ -0.04 $ & $ 0.01 $ & $ -0.05 $ & $ -0.06 $ \\ %the difference in part could be due to the inclusion of the strong dipole, and different numerical inputs
	%\hline
	\hline
	%NLO [Buras et al.] &
	$ m_c $ & $ 1.21 $ & $ -0.42 $ & $ 0.02 $ & $ -0.05 $ & $ 0.02 $ & $ -0.05 $ \\ %& --
	\hline
	%NLO [Buras et al.] &
	$   2 $~GeV & $ 1.14 $ & $ -0.31 $ & $ 0.009 $ & $ -0.03 $ & $ 0.01 $ & $ -0.03 $ \\ %& --
	\hline
	\end{tabular}
	%
	\\
	\vspace{0.5cm}
	%
	\begin{tabular}{|c|c|c|c|c|c|}
	\hline
	$ \mu $ & $ m_u $ & $ m_d $ & $ \hat{m} \equiv (m_u + m_d)/2 $ & $ m_s $ & $ m_c $ \\
	\hline\hline
	$ m_c $ & $2.50 \pm 0.09$ & $5.48 \pm 0.06$ & $ 4.00 \pm 0.06 $ & $109.0 \pm 0.7$ & $1280 \pm 13$ \\
	\hline
    $2$~GeV & $2.14 \pm 0.08$ & $4.70 \pm 0.05$ & $ 3.427 \pm 0.051 $ & $93.46 \pm 0.58$ & $1097 \pm 11$ \\
	%%$2$~GeV & $2.14 \pm 0.08$ & $4.70 \pm 0.05$ & $ 3.410 \pm 0.043 $ & \tp{$93.40 \pm 0.57$} %%% $93.44 \pm 0.68$ 
	%%& $1045 \pm 11$ \\
	\hline
	\end{tabular}
	\caption{\LVS{Wilson coefficients at NLO, in the NDR scheme, with four dynamical flavours \cite{Buchalla:1995vs}; $\Lambda^{(4)}_{\overline{\rm MS}} = 0.322$~GeV (which implies $ \alpha^{\rm NLO}_s (M_Z) = 0.1179 $), $ \mu_b = m_b $, with $m_b = 4.18$~GeV, and $M_W = 80.4$~GeV, $M_Z = 91.1876$~GeV, $m_t = 163.3$~GeV. The bottom panel gives the $ \overline{\text{MS}} $ quark masses in MeV at $ N_f = 2+1+1 $, see \cite{FlavourLatticeAveragingGroupFLAG:2021npn} and references therein; the running factor 0.857 for $m_c$ to $2$~GeV has been employed.}
	}\label{tab:WCs}
    %(we neglect the uncertainty in the latter running factor)
\end{table}

%the running factors $0.9026 (23)$ for $3$~GeV to $2$~GeV, and $0.7739 (60)$ for $3$~GeV to $m_c$, have been employed. \toni{The running factors are slightly outdated (see FLAG) and should be inverted. It doesn't make much sense to mention here 3 GeV. Better to give a single running factor from mc to 2 GeV (the error should be smaller than the combined one).}
%\LVS{I cross checked \href{http://flag.unibe.ch/2021/Media?action=AttachFile&do=get&target=FLAG_qmass.pdf}{FLAG2021} and the values seemed right; what reference are you using? OK, should be the version of February 2023}

==> table_amplitudes.tex <==
\begin{table}[h!]
\centering
\renewcommand{\arraystretch}{1.6}
	\begin{tabular}{|c||c|c|c|}
        \hline
		$ \delta^\pi_2 \simeq 0^{\rm o} $, $ \delta^K_1 \sim 115^{\rm o} $; & \multirow{2}{*}{nominal} & $ \text{Re} \{ \lambda_b \} = 0 $, & $ | \Omega_{11} | = | \Omega_{22} | = 1 $, \\
		$ \delta^\pi_2 \simeq \pm 180^{\rm o} $, $ \delta^K_1 \sim 115^{\rm o} $ & &  $ \text{Im} \{ \lambda_s \} = \text{Im} \{ \lambda_d \} = 0 $ & $ | \Omega_{12} | = | \Omega_{21} | = 0 $ \\
		\hline
		\hline
		$ \frac{\mathcal{B} ( D^0 \to \pi^+ \pi^-)_{theo;CV}}{\mathcal{B} ( D^0 \to \pi^+ \pi^-)_{exp;CV}} $ & $ 1.0 $ & id & $ 1.0 $; $ 1.0 $ \\
		$ \frac{\mathcal{B} ( D^0 \to \pi^0 \pi^0)_{theo;CV}}{\mathcal{B} ( D^0 \to \pi^0 \pi^0)_{exp;CV}} $ & $ 1.0 $ & id & $ 1.0 $; $ 0.8 $ \\
		$ \frac{\mathcal{B} ( D^+ \to \pi^+ \pi^0)_{theo;CV}}{\mathcal{B} ( D^+ \to \pi^+ \pi^0)_{exp;CV}} $ & fixed to 1 & id & id \\
		\hline
		$ A_{CP} ( D^0 \to \pi^+ \pi^-) \times 10^4 $ & $ 0.1 $; $ 3 $ & $ 0.4 $; $ 0.2 $ & $ 0.5 $; $ -0.4 $ \\
		$ A_{CP} ( D^0 \to \pi^0 \pi^0) \times 10^4 $ & $ 4 $; $ -1 $ & $ 0.1 $; $ 0.4 $ & $ -0.7 $; $ 1 $ \\
		$ A_{CP} ( D^+ \to \pi^+ \pi^0) $ & $ 0 $ & id & id \\
		\hline
		$ | \mathcal{A}^\pi_2 | \times 10^6 $ & $ 0.3 $ & id & id \\
		$ | \mathcal{A}^\pi_0 | \times 10^6 $ & $ 0.8 $ & id & id \\
		$ | \mathcal{B}^\pi_0 | / r_{\rm CKM} \times 10^6 $ & $ 0.4 $ & $ 0.03 $ & $ 0.8 $ \\
		%$ \arg(A^\pi_2) - \arg(A^\pi_0) $ & & & \\
		%$ \arg(A^\pi_0) - \arg(B^\pi_0) $ & & & \\
		$ \arg(\mathcal{A}^\pi_0) $ & $ 93^{\rm o} $ & id & $ 103^{\rm o} $ \\
		$ \arg(\mathcal{B}^\pi_0) $ & $ -74^{\rm o} $ & $ -50^{\rm o} $ & $ 103^{\rm o} - 180^{\rm o} = - 77^{\rm o} $ \\
		\hline
		$ \frac{\mathcal{B} ( D^0 \to K^+ K^-)_{theo;CV}}{\mathcal{B} ( D^0 \to K^+ K^-)_{exp;CV}} $ & $ 1.0 $ & id & $ 0.7 $ \\
		$ \frac{\mathcal{B} ( D^0 \to K_S K_S)_{theo;CV}}{\mathcal{B} ( D^0 \to K_S K_S)_{exp;CV}} $ & $ 1.0 $ & id & $ 0.7 $ \\
		$ \frac{\mathcal{B} ( D^+ \to K^+ K_S)_{theo;CV}}{\mathcal{B} ( D^+ \to K^+ K_S)_{exp;CV}} $ & fixed to 1 & id & id \\
		\hline
		$ A_{CP} ( D^0 \to K^+ K^-) \times 10^{4} $ & $ -1 $ & $ -0.2 $ & $ 0 $ \\
		$ A_{CP} ( D^0 \to K_S K_S) \times 10^{4} $ & $ -10 {\color{red} (-1)} $ & $ -2 $ & $ 0 $ \\
		$ A_{CP} ( D^+ \to K^+ K_S) $ & $ 0 $ & id & id \\
		\hline
		$ | \mathcal{A}^K_{11} | \times 10^6 $ & $ 0.6 \times f_1 $ & id & id \\
		$ | \mathcal{A}^K_{13} | \times 10^6 $ & sub-leading: $ N_c $ & id & id \\
		$ | \mathcal{A}^K_0 | \times 10^6 $ & $ 0.8 $ & id & $ 0.6 $ \\
		$ | \mathcal{B}^K_{11} | / r_{\rm CKM} \times 10^6 $ & $ 0.09 \times f_1 $ & $ 0.06 \times f_1 $ & $ 0.09 \times f_1 $ \\
		$ | \mathcal{B}^K_0 | / r_{\rm CKM} \times 10^6 $ & $ 0.4 $ & $ 0.04 $ & $ 0.09 $ \\
		%$ \arg(A^K_{11}) - \arg(A^K_0) $ & & & \\
		%$ \arg(A^K_0) - \arg(B^K_0) $ & & & \\
		$ \arg(\mathcal{A}^K_0) $ & $ -66^{\rm o} $ & id & $ -50^{\rm o} $ \\
		$ \arg(\mathcal{B}^K_0) $ & $ 99^{\rm o} $ & $ 73^{\rm o} $ & $ -50^{\rm o} $ \\
        \hline
	\end{tabular}
	\caption{Predictions based on the reference solution of Tab.~\ref{tab:num_sols_Omnes}. The notation $\mathcal{A}$ ($\mathcal{B}$) designates CP-even (respectively, CP-odd) amplitudes; ``id'' designates identical values up to the precision shown in the previous column along the same row, and ``CV'' stands for central value. {\color{red}[Ele: XCHECK]}}\label{tab:full_set_predictions}
    %[Note that for comparing the table with your CKMfitter results, you have to review the latter code!]
\end{table}

==> table_amplitudes_2.tex <==
\begin{table}[h!]
\centering
\renewcommand{\arraystretch}{1.6}
	\begin{tabular}{|c||c|c|c|}
        \hline
		$ \phi_2 \simeq 0^{\rm o} $, $ \phi_1 \sim 115^{\rm o} $; & \multirow{2}{*}{nominal} & $ | \Omega_{11} | = | \Omega_{22} | = 1 $, \\
		$ \phi_2 \simeq \pm 180^{\rm o} $, $ \phi_1 \sim 115^{\rm o} $ & & $ | \Omega_{12} | = | \Omega_{21} | = 0 $ \\
		\hline
		\hline
		$ \frac{\mathcal{B} ( D^0 \to \pi^+ \pi^-)_{theo;CV}}{\mathcal{B} ( D^0 \to \pi^+ \pi^-)_{exp;CV}} $ & $ 1.0 $ & id \\
		$ \frac{\mathcal{B} ( D^0 \to \pi^0 \pi^0)_{theo;CV}}{\mathcal{B} ( D^0 \to \pi^0 \pi^0)_{exp;CV}} $ & $ 1.0 $ & $ 1.0 $; $ 0.8 $ \\
		$ \frac{\mathcal{B} ( D^+ \to \pi^+ \pi^0)_{theo;CV}}{\mathcal{B} ( D^+ \to \pi^+ \pi^0)_{exp;CV}} $ & fixed to 1 & id \\
		\hline
		$ A_{CP} ( D^0 \to \pi^+ \pi^-) \times 10^4 $ & $ 0.1 $; $ 3 $ & $ 0.5 $; $ -0.4 $ \\
		$ A_{CP} ( D^0 \to \pi^0 \pi^0) \times 10^4 $ & $ 4 $; $ -1 $ & $ -0.7 $; $ 1 $ \\
		$ A_{CP} ( D^+ \to \pi^+ \pi^0) $ & $ 0 $ & id \\
		\hline
		$ | \mathcal{A}^\pi_2 | \times 10^6 $ & $ 0.3 $ & id \\
		$ | \mathcal{A}^\pi_0 | \times 10^6 $ & $ 0.8 $ & id \\
		$ | \mathcal{B}^\pi_0 | / r_{\rm CKM} \times 10^6 $ & $ 0.4 $ & $ 0.8 $ \\
		%$ \arg(A^\pi_2) - \arg(A^\pi_0) $ & & & \\
		%$ \arg(A^\pi_0) - \arg(B^\pi_0) $ & & & \\
		$ \arg(\mathcal{A}^\pi_0) $ & $ 93^{\rm o} $ & $ 103^{\rm o} $ \\
		$ \arg(\mathcal{B}^\pi_0) $ & $ -74^{\rm o} $ & $ 103^{\rm o} - 180^{\rm o} = - 77^{\rm o} $ \\
		\hline
		$ \frac{\mathcal{B} ( D^0 \to K^+ K^-)_{theo;CV}}{\mathcal{B} ( D^0 \to K^+ K^-)_{exp;CV}} $ & $ 1.0 $ & $ 0.7 $ \\
		$ \frac{\mathcal{B} ( D^0 \to K_S K_S)_{theo;CV}}{\mathcal{B} ( D^0 \to K_S K_S)_{exp;CV}} $ & $ 1.0 $ & $ 0.7 $ \\
		$ \frac{\mathcal{B} ( D^+ \to K^+ K_S)_{theo;CV}}{\mathcal{B} ( D^+ \to K^+ K_S)_{exp;CV}} $ & fixed to 1 & id \\
		\hline
		$ A_{CP} ( D^0 \to K^+ K^-) \times 10^{4} $ & $ -1 $ & $ 0 $ \\
		$ A_{CP} ( D^0 \to K_S K_S) \times 10^{4} $ & $ -10 $ & $ 0 $ \\
		$ A_{CP} ( D^+ \to K^+ K_S) $ & $ 0 $ & id \\
		\hline
		$ | \mathcal{A}^K_{11} | \times 10^6 $ & $ 0.6 \times |\Omega^{(1)}| $ & id \\
		$ | \mathcal{A}^K_{13} | \times 10^6 $ & sub-leading: $ N_c $ & id \\
		$ | \mathcal{A}^K_0 | \times 10^6 $ & $ 0.8 $ & $ 0.6 $ \\
		$ | \mathcal{B}^K_{11} | / r_{\rm CKM} \times 10^6 $ & $ 0.09 \times |\Omega^{(1)}| $ & id \\
		$ | \mathcal{B}^K_0 | / r_{\rm CKM} \times 10^6 $ & $ 0.4 $ & $ 0.09 $ \\
		%$ \arg(A^K_{11}) - \arg(A^K_0) $ & & & \\
		%$ \arg(A^K_0) - \arg(B^K_0) $ & & & \\
		$ \arg(\mathcal{A}^K_0) $ & $ -66^{\rm o} $ & $ -50^{\rm o} $ \\
		$ \arg(\mathcal{B}^K_0) $ & $ 99^{\rm o} $ & $ -50^{\rm o} $ \\
        \hline
	\end{tabular}
	\caption{Predictions based on the reference solution of Tab.~\ref{tab:num_sols_Omnes}. The notation $\mathcal{A}$ ($\mathcal{B}$) designates CP-even (respectively, CP-odd) amplitudes; ``id'' designates identical values up to the precision shown in the previous column along the same row, and ``CV'' stands for central value. When two numerical values are provided, the first corresponds to $ \phi_2 \simeq 0 $, while the second to $ \phi_2 \simeq \pm \pi $. {\color{red}[Ele: XCHECK no-rescattering \textbf{SHALL WE KEEP IT?}]}}\label{tab:full_set_predictions}
    %[Note that for comparing the table with your CKMfitter results, you have to review the latter code!]
\end{table}
